3DAC: Learning Attribute Compression for Point Clouds

We study the problem of attribute compression for large-scale unstructured 3D point clouds. Through an in-depth exploration of the relationships between different encoding steps and different attribute channels, we introduce a deep compression network, termed 3DAC, to explicitly compress the attributes of 3D point clouds and reduce storage usage in this paper. Specifically, the point cloud attributes such as color and reflectance are firstly converted to transform coefficients. We then propose a deep entropy model to model the probabilities of these coefficients by considering information hidden in attribute transforms and previous encoded attributes. Finally, the estimated probabilities are used to further compress these transform coefficients to a final attributes bitstream. Extensive experiments conducted on both indoor and outdoor large-scale open point cloud datasets, including ScanNet and SemanticKITTI, demonstrated the superior compression rates and reconstruction quality of the proposed 3DAC.

==> Tables/ablation_v0.tex <==


\begin{table}[htbp]
  \centering
  \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{cccccc|c}
    \Xhline{2.0\arrayrulewidth}
    \multicolumn{4}{c}{N}         & G & I & Birate \\
    d & w & l & a &       &       &  \\
    \hline
          &       &       &       &       &       & 3.85  \\
$\checkmark$ &       &       &       &       &       & 3.64  \\
$\checkmark$ & $\checkmark$ &       &       &       &       & 3.57  \\
$\checkmark$ & $\checkmark$ & $\checkmark$ &       &       &       & 3.51  \\
$\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ &       &       & 3.48  \\
$\checkmark$          &  $\checkmark$     &  $\checkmark$     &   $\checkmark$    &  $\checkmark$     &       & 3.28  \\
$\checkmark$          &  $\checkmark$     &  $\checkmark$     &   $\checkmark$    &   $\checkmark$    &  $\checkmark$     & 3.08  \\
          \Xhline{2.0\arrayrulewidth}
    \end{tabular}%
    }
    
\caption{Ablation study.}    
  \label{tab:query_layers}%
\end{table}%







% \begin{table}[htbp]
%   \centering
%   \resizebox{0.4\textwidth}{!}{
%     \begin{tabular}{cccccc|c}
%     \Xhline{2.0\arrayrulewidth}
%     \multicolumn{4}{c}{N}         & \multicolumn{1}{c}{\multirow{2}[0]{*}{G}} & \multicolumn{1}{c}{\multirow{2}[0]{*}{I}} & \multicolumn{1}{c}{\multirow{2}[0]{*}{Bitrate}} \\
%     \multicolumn{1}{l}{d} & \multicolumn{1}{l}{w} & \multicolumn{1}{l}{l} & \multicolumn{1}{l}{a} &       &       &  \\
%     \hline
%           &       &       &       &       &       & 3.846991 \\
%           &       &       &       &       &       & 3.639217 \\
%           &       &       &       &       &       & 3.572975 \\
%           &       &       &       &       &       & 3.506643 \\
%           &       &       &       &       &       & 3.483361 \\
%           &       &       &       &       &       & 3.27737 \\
%           &       &       &       &       &       & 3.075361 \\
%           \Xhline{2.0\arrayrulewidth}
%     \end{tabular}%
%     }
%   \label{tab:query_layers}%
% \end{table}%



% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{rrrrrr|r}
%     \multicolumn{4}{c}{N}         & \multicolumn{1}{c}{\multirow{2}[3]{*}{G}} & \multicolumn{1}{c|}{\multirow{2}[3]{*}{I}} & \multicolumn{1}{c}{\multirow{2}[3]{*}{Bitrate}} \\
% \cmidrule{1-4}    \multicolumn{1}{l|}{d} & \multicolumn{1}{l|}{w} & \multicolumn{1}{l|}{l} & \multicolumn{1}{l}{a} &       &       &  \\
%     \midrule
%           &       &       &       &       &       & 3.85  \\
%           &       &       &       &       &       & 3.64  \\
%           &       &       &       &       &       & 3.57  \\
%           &       &       &       &       &       & 3.51  \\
%           &       &       &       &       &       & 3.48  \\
%           &       &       &       &       &       & 3.28  \\
%           &       &       &       &       &       & 3.08  \\
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%







% \begin{table}[t]
% \centering
% \resizebox{0.4\textwidth}{!}{%
% \begin{tabular}{ccc|c}
% \Xhline{2.0\arrayrulewidth}
% N & G & I & Bitrate\\ 
% \hline
%   &  &  & 48.66\\
% $\checkmark$ &  &  & 48.66  \\
% $\checkmark$ & $\checkmark$ &  & 70.76\\
% $\checkmark$ & $\checkmark$ & $\checkmark$ & 54.21 \\

% \Xhline{2.0\arrayrulewidth}
% \end{tabular}%
% }
% \caption{Ablations of different levels of semantic query.}
% \label{tab:query_layers}
% \end{table}


% % Semantic3D
% \begin{table}[thb]
% \centering
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{c|rcccc}
% \Xhline{2\arrayrulewidth}
%  &  & \multicolumn{2}{c}{\textit{Semantic8}} & \multicolumn{2}{c}{\textit{Reduced8}} \\ 
%  & Methods & OA(\%) & \textbf{mIoU(\%)} & OA(\%) & \textbf{mIoU(\%)} \\
% \hline
% \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Full\\ sup.\end{tabular}} 
%  & SnapNet \cite{snapnet} & 91.0 & 67.4 & 88.6 & 59.1 \\
%  & PointNet++ \cite{qi2017pointnet++} & 85.7 & 63.1 & - & - \\ 
%  & ShellNet \cite{zhang2019shellnet} & - & - & 93.2 & 69.3 \\
%  & GACNet \cite{GACNet} & - & - & 91.9 & 70.8 \\
%  & RGNet \cite{RGNet} & 90.6 & 72.0 & 94.5 & 74.7 \\
%  & SPG \cite{landrieu2018large} & 92.9 & 76.2 & 94.0 & 73.2 \\
%  & KPConv \cite{thomas2019kpconv} & - & - & 92.9 & 74.6 \\
%  & ConvPoint \cite{boulch2020lightconvpoint} & 93.4 & 76.5 & - & - \\
%  & WreathProdNet \cite{wang2020equivariant} & 94.6 & \uline{77.1} & - & - \\
%  & RandLA-Net \cite{hu2019randla} & \uline{95.0} & 75.8 & \uline{94.8} & \uline{77.4} \\
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Weak\\ sup.\end{tabular}} 
%  %& \textbf{\nicknamenew{} (1\%)} & \textbf{95.2} & 76.2 & 94.6 & 76.0 \\
%  & \textbf{\nicknamenew{} (1\textperthousand)} & \textbf{94.8} & \textbf{72.3} & \textbf{93.7} & \textbf{74.7} \\
%  & \textbf{\nicknamenew{} (1‱)} & 91.9  & 58.8 & 90.3 & 65.6 \\
%  \Xhline{2.0\arrayrulewidth}
% \end{tabular}%
% }
% \caption{Quantitative results of different approaches on Semantic3D \cite{Semantic3D}. The scores are obtained from the recent publications. Accessed on 17 March 2021.}
% \label{tab:Semantic3D}
% \end{table}








==> chapters/010_intro_0903.tex <==

Recent progress in 3D sensing and capturing technology has enabled acquisition of large-scale point cloud scenes. Typically, one point cloud frame often contains from millions to billions of points. This huge amount of point cloud data in the raw format brings challenges to both efficient storage and transmission. In order to deal with this problem, point cloud compression is necessary.


Recently, several works [] show that point cloud deep compression is a promising research domain. For example, inspired by 2D image deep compression, Wang \textit{et al.} [] voxelized the point cloud first and proposed a 3D auto-encoder based method to reconstruct the point cloud geometry. In [], they constructed an octree to reorganize the raw point cloud data and develop corresponding deep entropy models for entropy coding[]. However, most works only focus on point cloud geometry compression and the compression of point cloud attributes (\textit{e.g.}, color, reflectance) is still a significant problem for our deep learning and compression community. For instance, when using MPEG’s standard point cloud compression method (G-PCC) [], the compressed colors bitstream accounts for 10\% to 60\% of the total bitstream for lossy geometry and lossy attribute compression and 90\% for lossless geometry and lossless attribute compression under the official configuration. 

% to do, transform based related work



\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/teaser/teaser.pdf}
	\end{center}
    \caption{Qualitative results of 3D Auto-Encoder based method, G-PCC and our \nickname{} for point cloud attribute compression on the Scannet dataset. $\rm BPP$ denotes bits per point and $\rm PSNR_y$ denotes peak signal-to-noise ratio of the luminance component. \nickname{} achieve comparable or even better results than G-PCC especially at high BPP.}
	\label{fig:teaser}
\end{figure}





In this work, we focus on point cloud attribute compression and assume point cloud geometry (positions of points) has been transmitted. Intuitively, it seems possible to develop point cloud attribute compression through combining deep image compression and point cloud learning as wang[]. More specifically, a most naive method can be realized with three steps, 1) extract point cloud latent feature using a 3D auto-encoder, 2) quantize the latent feature and 3) learn a deep entropy model for entropy coding. Unfortunately, due to the high complexity of point cloud data, we find that relative low-quality reconstruction results are obtained even with extremely low compression rate as shown in Figure \ref{fig:teaser}. This indicates that most information is lost through the vanilla 3D auto-encoder so it is difficult to learn point cloud attribute information. 

% Thus, there are two challenges of point cloud attribute compression, realizing high-quality point cloud attribute reconstruction and developing a compatible deep entropy model.


% Thus, we believe the key of deep learning-based point cloud attribute compression is realizing high-quality point cloud attribute reconstruction and developing a compatible deep entropy model.



%motivation of 3D wavelet transform and entropy model, why 3D wavelet transform, the pros of 3D wavelet transform, to do.




\begin{figure*}[thb]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/method/method_network_arch.pdf}
	\end{center}
    \caption{The overview network architecture of the proposed method for point cloud attribute compression. }
	\label{fig:method_overview}
\end{figure*}



In this paper, we propose a point cloud attribute compression network based on 3D wavelet transform, namely \textbf{\nickname{}}. In order to ensure the attribute reconstruction quality, We first adopt an efficient 3D wavelet transform, region adaptive hierarchical transform (RAHT) []. Then we propse a learning-based entropy model and explore the prior and context feature based on both RAHT and the point cloud data for our deep entropy model. In addition, to reduce the redundancy between different attribute channels, a inter channel prediction module is also included. As shown in Figure \ref{fig:teaser}, our wavelet-based approach achieves competitive results compared with 3D auto-encoder based compression method and MPEG’s standard point cloud compression method.





Our main contributions of this paper are as follows:
\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{1pt}
\setlength{\parsep}{1pt}
\setlength{\parskip}{1pt}
    \item We propose a learning-based point cloud attribute compression method leveraging 3D wavelet transform. 
    \item We adopt various context to the deep entropy model for point cloud attribute compression. 
    \item Our approach achieves the state-of-the-art compression performance on both indoor and outdoor datasets for the task of point cloud attribute compression.
\end{itemize}



==> chapters/010_intro_1102.tex <==



% point cloud compression, attribute compression
%Point clouds have been widely used in various applications such as mixed reality, self-driving vehicles, and high-resolution mapping. With the rapid development of 3D acquisition technology, point clouds become increasingly accessible. The storage and transmission of a large amount of points become a challenging problem for these applications with massive point clouds. Except compression of points' 3D coordinates, attribute (\textit{e.g.}, color, reflectance) compression takes a large part in a practical point cloud compression system\footnote{For example, with the standard point cloud compression algorithm of MPEG (i.e., G-PCC \cite{schwarz2018emerging}), attribute compression takes up to 60\% and 90\% of the overall bitstream for lossy and lossless compression, respectively.}. It is therefore, highly necessary to develop effective and efficient attribute compression algorithms for point clouds.

\qy{As a common 3D data representation, point clouds have been widely used in a variety of real applications such as mixed reality, self-driving vehicles, and high-resolution mapping. Thanks to the remarkable progress achieved in 3D acquisition technology, point clouds become increasingly accessible recently. However, the storage and transmission of massive irregularly sampled points pose a new challenge to existing techniques. In particular, along with the raw 3D coordinates of each point, the compression of the corresponding point attributes (\textit{e.g.}, color, reflectance) is also non-trivial\footnote{For example, with the standard point cloud compression algorithm of MPEG (\textit{i.e.}, G-PCC \cite{schwarz2018emerging}), attribute compression takes up to 60\% and 90\% of the overall bitstream for lossy and lossless compression, respectively.}. In this regard, we will study the efficient attribute compression for unstructured point clouds in this paper.
}

% \cite{schwarz2018emerging}



% limitation of traditional entropy coding
% 1. traditional method of attribute compression
% 2. initial coding and entropy coding
% 3. limitation of entropy coding

% % to do: 
% 1. the motivation of entropy coding (information theory and probability). 
% 2. the limitation of traditional entropy coding, following the motivation.

% \cite{zhang2014point}

%Previous methods \cite{zhang2014point, thanou2015graph, shao2017attribute, shao2018hybrid, de2016compression, souto2020predictive, pavez2021multi, pavez2020region} usually adopt signal or image transforms on point cloud to achieve attribute compression. These methods typically contain two steps, initial coding of attribute and entropy coding of transformed coefficients. In the initial coding stage, signal processing techniques, such as graph Fourier transform \cite{zhang2014point} and wavelet transform \cite{de2016compression}, are adopted to convert point cloud attributes to specific domain coefficients. These approaches successfully process unstructured and large-scale point clouds and ensure the reconstruction quality with the help of the mature signal processing techniques. According to the information theory, a lower bound of bitrate can be further achieved by an entropy coder given the actual distribution of the transmitted coefficients. Thus, entropy coding is futher conducted to compress the transformed and quantized coefficients to the final bitstream. However, less attention is paid on this part, and only a few entropy coders based on Run-Length and arithmetic coders \cite{malvar2006adaptive, gu20193d, schwarz2018emerging} are developed and used for attribute compression. These traditional hand-crafted entropy coders take coefficients as a sequence of symbols and estimate the distribution only considering the previous input symbols as context information. Intuitively, deep neural networks have a stronger ability to predict the distribution according to data priors and much more complicated context information.

To achieve effective attribute compression of 3D point clouds, early works \cite{zhang2014point, thanou2015graph, shao2017attribute, shao2018hybrid, de2016compression, souto2020predictive, pavez2021multi, pavez2020region} usually resort to signal or image transforms on 3D point clouds. In general, these methods follow a two-step framework, \textit{i.e.}, the initial coding of attributes and entropy coding of transformed coefficients. In the initial coding stage, signal processing techniques such as graph Fourier transform \cite{zhang2014point} or wavelet transform \cite{de2016compression} is usually leveraged to convert the unstructured and large-scale point cloud attributes to a number of specific domain coefficients. Next, coefficients are quantized and entropy coded to generate the final bitstream\footnote{According to the information theory \cite{shannon1948mathematical}, a lower bound of bitrate can be further achieved by an entropy coder given the actual distribution of the transmitted coefficients.}. A handful of entropy coders based on Run-Length and arithmetic coders \cite{malvar2006adaptive, gu20193d, schwarz2018emerging} are developed for attribute compression. These traditional hand-crafted approaches take coefficients as a sequence of symbols and estimate the distribution only considering the previous input symbols as context information. In general, these aforementioned entropy coders do not consider geometry information of point clouds and designed independently with the initial coding methods. Furthermore, these methods are not able to effectively utilize attributes correlations within each channel.






\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/teaser/teaser_final.pdf}
	\end{center}
    %\caption{Qualitative results of 3D Auto-Encoder based method, G-PCC and our \nickname{} for point cloud attribute compression on the Scannet dataset. $\rm BPP$ denotes bits per point and $\rm PSNR_y$ denotes peak signal-to-noise ratio of the luminance component. \nickname{} achieves comparable or even better results than G-PCC especially at high bitrates.}
    \caption{\qy{Qualitative point cloud attribute compression results of 3D auto-encoder based method, G-PCC and our \nickname{} on the ScanNet \cite{scannet} dataset. Bits Per Point (BPP) and Peak Signal-to-Noise Ratio (PSNR) of the luminance component are also reported. Note that, the raw point clouds usually use uint8 RGB values (\textit{i.e.,}  $8\times3=24$ BPP).}}

	\label{fig:teaser}
\end{figure}

\begin{figure*}[thb]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/method/method_network_arch.pdf}
	\end{center}
    \caption{The network architecture of our point cloud attribute compression method. }
	\label{fig:method_overview}
\end{figure*}






Recent deep neural network based entropy models show their ability in entropy coding. Prior approaches \cite{huang20193d, quach2019learning, wang2021multiscale} extended image auto-encoders and deep entropy models to point cloud geometry compression. However, they are not readily extend to attribute compression due to the failure in attribute reconstruction as shown in Fig. \ref{fig:teaser}. Other recent works \cite{huang2020octsqueeze, biswas2020muscle, que2021voxelcontext} adopted octree-structure entropy models for point cloud compression. They extracted context feature highly based on their initial coding method (octree coding) in order to explore the redundancies within the occupancy symbols. These methods mainly focus on geometry compression and do not apply specific technique for attribute compression. It is possible to boost attribute compression performance through combining mature initial coding method with a task-specific deep entropy model.







%In this paper, we propose a learning based method for point cloud attribute compression. We first adopt a point cloud attribute transform, Region Adaptive Hierarchical Transform (RAHT) \cite{de2016compression}, to convert point cloud attributes to frequency-domain coefficients. Then, we introduce a learning based entropy model by exploiting context information highly based on the initial coding stage and the inter channel correlation.  As shown in Fig. \ref{fig:teaser}, our method achieves better results than the 3D auto-encoder based compression method and the standard point cloud compression method in MPEG \cite{schwarz2018emerging}.

\qy{In this paper, we propose a learning-based method for point cloud attribute compression. In particular, for initial coding, the Region Adaptive Hierarchical Transform (RAHT) \cite{de2016compression} is first adopted to transform point cloud attributes to coefficients. We then introduce a learning-based entropy model to estimate the probability distribution of transformed coefficients by exploiting the rich context information hidden in the initial coding method (i.e. RAHT) and the inter-channel correlation. As shown in Fig. \ref{fig:teaser}, our method achieves better results than the vanilla 3D auto-encoder-based compression method and the standard point cloud compression method in MPEG \cite{schwarz2018emerging}.}


%to do

%这里总结的前两个创新点依然不够吸引人，我们在后续的修改中再不断优化。
\qy{To summarize, the main contributions of this paper are as follows:}
\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{1pt}
\setlength{\parsep}{1pt}
\setlength{\parskip}{1pt}
    % \item We propose a learning-based point cloud attribute compression method with 3D wavelet transform. 
    % \item We introduce a deep entropy model using the context information extracted from both the data after wavelet transform and the original point cloud.
    % \item Our approach achieves the state-of-the-art point cloud attribute compression performance on both indoor and outdoor datasets.
    \item \qy{We propose a learnable point cloud attribute compression method with 3D wavelet transform. }
    \item \qy{We introduce a deep entropy model to exploit the input-level and latent-feature level context in the raw point clouds and the feature map after wavelet transform, respectively.}
    \item \qy{Extensive experiments conducted on both indoor and outdoor datasets demonstrated the state-of-the-art point cloud attribute compression performance of the proposed \nickname{}.}
\end{itemize}





==> chapters/010_intro_v0.tex <==

\gary{Point clouds have been widely used in various applications such as mixed reality, self-driving vehicles, and high-resolution mapping. With the rapid development of 3D acquisition technology, point clouds become increasingly accessible. The storage and transmission of a large amount of points become a challenging problem for these applications with massive point clouds. Consequently, point cloud compression is highly required.}

%Recent progress in 3D acquisition makes large-scale point clouds available. Typically, one point cloud frame often contains from millions to billions of points. This huge amount of point cloud data in the raw format brings challenges to both efficient storage and transmission. In order to deal with this problem, point cloud compression is necessary.

\gary{Existing point cloud compression methods can broadly be categorized into geometry compression and attribute compression methods \cite{}. The task of geometry compression is to compress the 3D coordinates of points, while the task of attribute compression is to compress the attributes (\textit{e.g.}, color, reflectance) of points. Although a large number of traditional methods have been proposed in the last two decades, they still face several challenges. First, since these methods usually achieve point cloud compression with two independent steps: initial coding (\textit{e.g.}, with graph transform [], wavelet transform []) and entropy coding, the context information from the initial coding step cannot be used to benefit the entropy coding step. Second, data priors (such as point cloud geometry) are also ignored \TBD{during attribute compression} \cite{}. Third, most of these hand-crafted methods are developed for dense point clouds, leading to performance degradation on sparse point clouds (e.g., acquired by LiDARs).}


%Traditional methods usually achieve point cloud compression following the pipeline of image compression. Data priors and contextual information is ignored due to the limitations of the hand-crafted methods.




% GC: please list the of limits of traditional point cloud compression methods that can be addressed by DL.
% limitations of traditional methods/hand-crafted  methods:
% 1. Most traditional methods are developed based on dense point cloud (overfitting?). Our method performs better on Semantic KITTI rather than ScanNet.
% 2. Traditional methods follow the pipeline of traditional image compression. The initial coding step and the entropy coding step are independent.
% 3. Data prior (geometry prior) is not utilized.

\gary{Recently, deep learing approaches have been investigated to achieve point cloud compression.
For example, a 3D auto-encoder with deep entropy \cite{} and octree-based entropy models \cite{} are proposed to improve the point cloud compression performance. However, these methods mainly focus on geometry compression, while deep learning based attribute compression is still in its infancy. Meanwhile, attribute compression takes a large part in a practical point cloud compression system\footnote{For example, with the standard point cloud compression algorithm of MPEG (i.e., G-PCC), attribute compression takes up to 60\% and 90\% of the overall bitstream for lossy and lossless compression, respectively.}. %, which consists of both geometry compression and attribute compression. 
It is therefore, highly necessary to develop effective and efficient attribute compression algorithms for point clouds with deep learning.}

%接下来这段，应该是描述点云属性压缩面临的挑战和困难，或者现有点云属性压缩依然没有做好的问题，这些挑战和困难要能能本文所要解决的问题对应上。也要能引出来为什么在本文中要先用RAHT？你先重写一下，我再接着改。

%Recent works [] show that point cloud deep compression is a promising research domain. Wang [] adopted a 3D auto-encoder with deep entropy model and Huang [] used octree-based entropy models to improve the compression performance. Most works only focus on point cloud geometry compression, while the compression of point cloud attributes (\textit{e.g.}, color, reflectance) is still a significant problem for our deep learning and data compression community. For instance, when using MPEG’s standard point cloud compression method (G-PCC) [], the compressed colors bitstream accounts for 10\% to 60\% of the total bitstream for lossy geometry and lossy attribute compression and around 90\% for lossless geometry and lossless attribute compression under the official configuration. 






% to do, transform based related work


\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/teaser/teaser.pdf}
	\end{center}
    \caption{Qualitative results of 3D Auto-Encoder based method, G-PCC and our \nickname{} for point cloud attribute compression on the Scannet dataset. $\rm BPP$ denotes bits per point and $\rm PSNR_y$ denotes peak signal-to-noise ratio of the luminance component. \nickname{} achieves comparable or even better results than G-PCC especially at high bitrates.}
	\label{fig:teaser}
\end{figure}


% More specifically, a most naive method can be realized with three steps, 1) extract point cloud latent feature using a 3D auto-encoder, 2) quantize the latent feature and 3) learn a deep entropy model for entropy coding. 



% Some works [] used graph transform to decompose point cloud attributes to coefficients which are then quantized and entropy coded. Although these methods are able to achieve decent compression performance, they are not practical because of the high computing complexity.



%接下来这段，应该是描述点云属性压缩面临的挑战和困难，或者现有点云属性压缩依然没有做好的问题，这些挑战和困难要能能本文所要解决的问题对应上。也要能引出来为什么在本文中要先用RAHT？你先重写一下，我再接着改。



%Traditional methods usually achieve point cloud compression with the initial coding (\textit{e.g.}, graph transform [], wavelet transform []) and an entropy coder independently. Thus, the contextual information from the initial coding step is not able to benefit the entropy coding. Data priors including point cloud geometry are also ignored. Moreover, most of these hand-crafted methods are developed based on dense point clouds leading to performance degradation on sparse point clouds, such as lidar scans.


\gary{Previous methods usually utilize signal processing techniques to achieve point cloud attribute compression. 
Queiroz [] adopted Region Adaptive Hierarchical Transform (RAHT) to decompose attributes into low-frequency and high-frequency coefficients, which are then quantized and entropy coded. This method takes the advantage of traditional data reconstruction and compression techniques, while ignores the redundant information in the initial coding and the entropy coding stages.}
%The redundancy can further be exploited to improve the compression performance. 
%comments: 数据先验和前文中的数据冗余性之间是什么样的关系？逻辑流能跟流畅一点会更好。
With strong priors in the signal and geometry domain, context information from the initial coding (\textit{e.g.}, relation between decomposed coefficients) and the point cloud geometry can further be exploited to reduce the data redundancy, thus improving the compression performance. \gary{In the area of image compression, it is already demonstrated that deep learning based methods, such as the probability density model [], are able to learn data priors. However, a 3D auto-encoder tends to learn low-frequency information but ignores high-frequency information, leading to poor attribute reconstruction performance (as shown in Fig. \ref{fig:teaser}).}


% redundancy 
% 1. context information from the initial coding. for example, low- and high-frequency coefficients of RAHT
% 2. point cloud geometry. similar local pattern, similar attribute
% 3. redundancy between inter channel attributes. predict green channel from red.









%point cloud attribute compression prefer signal processing techniques for attribute reconstruction. Queiroz [] adopted a variant of Haar wavelet transform, Region Adaptive Hierarchical Transform (RAHT), to decompose attributes to low- and high-frequency coefficients which are then quantized and entropy coded. This method takes advantage of traditional data reconstruction and compression techniques, while it ignores the redundant information behind the initial coding and the entropy coding stage. This redundancy can be further exploit to improve the compression performance. In contrast, popular deep image compression methods, probability density model [], have the capability of learning data priors. However, we observe that the 3D auto encoder tends to learn low-frequency information and ignore the high-frequency part, leading to failure of attribute reconstruction as shown in Figure \ref{fig:teaser}.




%%In this work, we focus on point cloud attribute compression and assume that point cloud geometry (positions of points) has been transmitted. Intuitively, it seems possible to develop point cloud attribute compression through combining deep image compression and point cloud learning. More specifically, use a 3D auto-encoder for attribute reconstruction and a deep entropy model for entropy coding. Unfortunately, due to the high complexity of the point cloud data, we find that relative low-quality reconstruction results are obtained even with an extremely low compression rate as shown in Figure \ref{fig:teaser}. This indicates that most information is lost through a vanilla 3D auto-encoder so it finds difficult to preserve point cloud attribute information. In contrast, traditional point cloud attribute compression methods [] prefer signal processing techniques for attribute reconstruction. Queiroz [] adopted a variant of Haar wavelet transform to decompose attributes to low- and high-frequency coefficients which are then quantized and entropy coded. This method takes advantage of traditional data reconstruction and compression techniques, while it ignores the redundant information behind the wavelet coefficients during entropy coding.



% Transform-based methods [] adopt signal processing techniques to transform point cloud attribute to corresponding coefficients 

% Thus, there are two challenges of point cloud attribute compression, realizing high-quality point cloud attribute reconstruction and developing a compatible deep entropy model.

% Thus, we believe the key of deep learning-based point cloud attribute compression is realizing high-quality point cloud attribute reconstruction and developing a compatible deep entropy model.

%motivation of 3D wavelet transform and entropy model, why 3D wavelet transform, the pros of 3D wavelet transform, to do.




\begin{figure*}[thb]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/method/method_network_arch.pdf}
	\end{center}
    \caption{The network architecture of our point cloud attribute compression method. }
	\label{fig:method_overview}
\end{figure*}

\gary{In this paper, we propose a deep neural network (namely, {\nickname{}}) for point cloud attribute compression. %with 3D wavelet transform and a point-based deep neural network. 
To achieve high quality of attribute reconstruction, we first adopt the RAHT method \cite{} to perform initial coding of point cloud attributes. Then, we extract context information from the RAHT step and the point cloud, and propose a learning-based entropy model. We further introduce an inter-channel prediction module to reduce the redundancy within multiple attribute channels. As shown in Fig. \ref{fig:teaser}, our method achieves better results than the 3D auto-encoder based compression method \cite{} and the standard point cloud compression method in MPEG \cite{}.}

%这里总结的前两个创新点依然不够吸引人，我们在后续的修改中再不断优化。
\gary{The main contributions of this paper are as follows:
\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{1pt}
\setlength{\parsep}{1pt}
\setlength{\parskip}{1pt}
    \item We propose a learning-based point cloud attribute compression method with 3D wavelet transform. 
    \item We introduce a deep entropy model using the context information extracted from both the data after wavelet transform and the original point cloud.
    \item Our approach achieves the state-of-the-art point cloud attribute compression performance on both indoor and outdoor datasets.
\end{itemize}
}


==> chapters/020_related_0928.tex <==

% Point Cloud Compression

\subsection{Point Cloud Compression}

Existing point cloud compression methods can broadly be categorized into geometry compression and attribute compression methods. The task of geometry compression is to compress the 3D coordinates of points, while the task of attribute compression is to compress the attributes (\textit{e.g.}, color, reflectance) of points.

For point cloud geometry compression, most approaches [] adopted an octree to organize the raw point cloud data. For example, G-PCC [] includes a octree-based method for geometry compression. Recently, several learning based methods \cite{huang2020octsqueeze, biswas2020muscle, que2021voxelcontext} also applied the octree structure for initial coding. Other methods \cite{huang20193d, yan2019deep, quach2019learning, quach2020improved, wang2021multiscale} extended the deep entropy model \cite{balle2018variational} to 3D domain with 3D auto encoders.

Most attribute compression approaches apply traditional signal or image transforms on point cloud data. Zhang et al. \cite{zhang2014point} splited point cloud as blocks through octree and used graph Fourier transform, and Thanou et al. \cite{thanou2015graph} extended this work to dynamic attribute compression. Shao et al. \cite{shao2017attribute, shao2018hybrid} organized point cloud as kd-tree and also adopted graph transform. Queiroz et al. \cite{de2016compression} proposed a variant of Haar wavelet transform, namely region-adaptive Haar transform (RAHT), to decompose attributes into low- and high-frequency coefficients. Several works are developed based on RAHT with intra- and inter-frame prediction \cite{souto2020predictive, pavez2021multi}, graph transform \cite{pavez2020region} and fixed-point operations \cite{sandri2019integer}. 





\subsection{Entropy Coders for Data Compression}





\subsection{Point Cloud Geometry Compression}\label{sec:sup_nets}
%comments：这里不是introduction，需要对主要的方法一两句话展开评述（一句话描述基本思路和方法，一句话描述优缺点）。因此，这部分需要扩充下篇幅。你参考下往年CVPR论文的主流写法。这里一点都不要提到本文的工作，但在介绍现有工作的时候，其指向性要很明确，就是为了引出我们自己的工作。
Recently, several deep learning based point cloud geometry compression methods have been proposed. One class of these methods \cite{huang20193d, yan2019deep, quach2019learning, quach2020improved, wang2021multiscale} adopted various 3D auto encoders to reconstruct the point cloud geometry and a probability density model \cite{balle2018variational} for entropy coding. Existing point-based or voxel-based neural netowrks \cite{huang20193d, yan2019deep, quach2019learning, quach2020improved} are adopted for point cloud encoding. A sparse convolution based autoencoder \cite{wang2021multiscale} is also included for point cloud compression and reconstruction. However, we observe that 3D auto encoders fail in attribute reconstruction. Other methods \cite{huang2020octsqueeze, biswas2020muscle, que2021voxelcontext} organized point cloud as an octree and then develop octree-structured entropy models. Inspired by these methods, we aims to develop a deep entropy model for attribute compression.



\subsection{Point Cloud Attribute Compression}
Point cloud attribute compression methods can be roughly categorized as LODs (Levels of Details) based methods \cite{huang2008generic, schnabel2006octree, waschbusch2004progressive, huang2021hierarchical} and transform based method \cite{zhang2014point, thanou2015graph, shao2017attribute, shao2018hybrid, de2016compression, souto2020predictive, pavez2021multi, pavez2020region, sandri2019integer}. LODs based methods usually decompose point cloud into multiple LODs, then predict and encode the attributes based on LODs. Transform based methods adopt traditional signal or image transforms on point cloud data. Zhang et al. \cite{zhang2014point} applied graph transform to the octree and used arithmetic coding for intra-frame attribute compression, and Thanou et al. \cite{thanou2015graph} extended this work to inter-frame compression. Shao et al. \cite{shao2017attribute, shao2018hybrid} organized point cloud as kd-tree and then adopted graph transform. Queiroz et al. \cite{de2016compression} proposed a more efficient transform based method compared with previous methods.A variant of Haar wavelet transform, namely region-adaptive Haar transform (RAHT), was applied to octree instead of graph transform. Several works are developed based on RAHT with intra- and inter-frame prediction \cite{souto2020predictive, pavez2021multi}, graph transform \cite{pavez2020region} and fixed-point operations \cite{sandri2019integer}. Deep learning is not adopted by all of these methods.



















% \textbf{Point Cloud Geometric Compression.}

% \textbf{Point Cloud Attribute Compression.} 


% Deep Image and Video Compression
%\subsection{Deep Image Compression}









% 1. geometry compression, not attribute
% 2. transform based method, no deep learning
% 3. image compression, can not extend to 3D domain




==> chapters/020_related_v1.tex <==

\subsection{Point Cloud Compression}




\qy{Existing works on 3D point cloud compression are mainly focused on two aspects: geometry compression and attribute compression. By definition, geometry compression aims to compress the 3D coordinates of points, while the objective of attribute compression is to compress the attributes (\textit{e.g.}, color, reflectance) of points.}

\qy{\textbf{Geometry compression.} In light of the unstructured nature of 3D point clouds, existing methods  \cite{meagher1982geometric, schwarz2018emerging} usually leverage the advanced data structure such as octree to organize the raw point clouds. For example, G-PCC \cite{schwarz2018emerging} includes an octree-based method for geometry compression. Later, several learning-based approaches \cite{huang2020octsqueeze, biswas2020muscle, que2021voxelcontext} also applied the octree structure for initial coding. In addition, several methods \cite{huang20193d, yan2019deep, quach2019learning, quach2020improved, wang2021multiscale} extended the deep entropy model \cite{balle2018variational} to 3D domain with 3D autoencoders. However, due to the high complexity of point cloud attributes, it is infeasible to extend this framework to attribute compression.}



\qy{\textbf{Attribute compression.} The general idea to achieve point clouds attribute compression is to apply traditional signal or image transforms. Specifically, Zhang et al. \cite{zhang2014point} first split point cloud as blocks through Octree and used graph Fourier transform, and Thanou et al. \cite{thanou2015graph} extended this work to dynamic attribute compression. Shao et al. \cite{shao2017attribute, shao2018hybrid} organized point cloud as KD-Tree structure and also adopted graph transform. Due to the repeated eigendecomposition, graph transform-based methods are usually time-consuming. To deal with this problem, Queiroz et al. \cite{de2016compression} proposed a variant of Haar wavelet transform, namely region-adaptive Haar transform (RAHT) for real-time point cloud transmission. Several follow up works further extended RAHT with intra- and inter-frame prediction \cite{souto2020predictive, pavez2021multi}, graph transform \cite{pavez2020region} and fixed-point operations \cite{sandri2019integer}. A handful of recent works started to explore deep learning techniques for point cloud attribute compression. Maurice et al. \cite{quach2020folding} used FoldingNet \cite{yang2018foldingnet} to reorganize the input point cloud as an image and then compressed it with a conventional 2D image codec. MuSCLE \cite{biswas2020muscle} toke the quantized point cloud intensity as symbols and extracted spatio-temporal information for entropy coding. However, it remains challenging for these methods to achieve low bitrates as well as preserve reconstruction quality without exploring the information reduancy hidden in data.}




to do: merge this part to point cloud compression and image compression



%\cite{goyal2018deepzip}
\subsection{Entropy Coding for Data Compression}



\qy{Traditional entropy coding aims to model the real probability distribution of symbols based on hand-crafted techniques, and encodes symbols with the estimated distribution through the entropy coder, such as Huffman \cite{huffman1952method}, arithmetic \cite{witten1987arithmetic} and Golomb-Rice coders \cite{weinberger2000loco, richardson2004h}. In \cite{zhang2014point, de2017transform}, they assumed that the transmitted symbols follow a certain Laplacian distribution and then encode them with arithmetic coding. However, the estimated distribution is usually difficult to approximate the real distribution due to the naive assumption. In \cite{de2016compression, souto2020predictive, pavez2021multi}, an adaptive run-length Golomb-Rice (RLGR) coder \cite{malvar2006adaptive} was adopted for entropy coding. Variants of run-length coding were also adopted by \cite{schwarz2018emerging, gu20193d}. All of these entropy coders take input symbols as sequential data and only adjust their encoding parameters depending on the previous input symbols.
}




\qy{Deep learning-based entropy coders tend to predict symbol distribution based on data prior and context information. Goyal et al. and Chandak et al. \cite{goyal2018deepzip, chandak2020lfzip} adopted a recurrent neural network to achieve sequential data compression through aggregating context features from encoded symbols. Ball{\'e} et al. \cite{balle2016end, balle2018variational} proposed fully factorized models to estimate the probability distribution of latent features. For point cloud geometry compression, Huang et al. \cite{huang2020octsqueeze} encoded raw point cloud data as an octree and proposed an octree-based deep entropy model. Biswas et al. \cite{biswas2020muscle} and Que et al. \cite{que2021voxelcontext} also followed the octree structure, and aggregated spatio-temporal and voxel context feature into the deep entropy model respectively. However, these octree-based entropy coders are highly geometry compression-oriented. In particular, Muscle \cite{biswas2020muscle} is proposed for LiDAR intensity compression, and only considers the LiDAR geometry and intensity of the previous frame. The compression performance can be further improved by incorporating the context information from the current frame, or exploiting context information from other point cloud data structures and initial coding methods.}




\subsection{Deep Image Compression}

The traditional image compression \cite{wallace1992jpeg, goyal2001theoretical, skodras2001jpeg, sullivan2012overview, bpg} typically contains three steps inlcuding transformation, quantization and entropy coding. In particular, the source image is first transformed from signal domain to certain frequency domain, to capture spatial redundancy as well as representing raw data with a few transformed coefficients. These coefficients are then quantized with a hand-crafted quantization table and entropy coded for further compression. For example, the well-known JPEG standard adopted discrete cosine transform on image blocks for transformation, and differential pulse code modulation and run length coding with Huffman coding for entropy coding of DC and AC coefficients respectively \cite{wallace1992jpeg}. Different from JPEG, JPEG2000 adopted discrete wavelet transform and an arithmetic coder \cite{goyal2001theoretical, skodras2001jpeg}, and has a superior compression performance compared with JPEG.


In contrast to traditional image compression approaches, deep learning based methods jointly optimize the three steps. Most recent methods \cite{balle2016end, balle2018variational, yang2021slimmable, he2021checkerboard, deng2021deep, gao2021neural, bai2021learning} adopt an auto-encoder architecture. These methods formulate a nonlinear function with a encoder to map source image to a more compressible latent space and recover the image from the latent codes with a decoder. Then, they model the entropy of the latent codes as a tight lower bound of the bitrate also with separate neural networks. Specifically, Ball{\'e} et al. \cite{balle2016end} used convolution neural networks to model both the non-linear transform and the entropy model, and encoded side information for better entropy modelling in their following work \cite{balle2018variational}. Deng et al. \cite{deng2021deep} extended the architecture to stereo image compression with homography transformation and well-designed entropy models.







==> chapters/030_method_1106.tex <==


\begin{figure*}[thb]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/method/method_network_arch.pdf}
	\end{center}
    \caption{The network architecture of our point cloud attribute compression method. }
	\label{fig:method_overview}
\end{figure*}



\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/method/method_raht.pdf}
	\end{center}
    \caption{An illustration of RAHT and RAHT tree. (a) A 2D example of RAHT, (b) The corresponding RAHT tree.}
	\label{fig:method_raht}
\end{figure}


% \begin{figure}[t]
% 	\begin{center}
% 		\includegraphics[width=1.0\linewidth]{Figures/method/method_sparse_conv_net.pdf}
% 	\end{center}
%     \caption{SparseConvNet for RAHT tree nodes feature extraction. TBD{move to appendix}}
% 	\label{fig:method_sparse_conv_net}
% \end{figure}






% Overview
\subsection{Overview}

\qy{Given large-scale 3D point clouds, this paper mainly focuses on the task of point cloud attribute compression, and geometry of point clouds is assumed to have been separately transmitted. As depicted in Fig. \ref{fig:method_overview}, our framework is composed of an initial coding-based and inter-channel-based context module with a learning-based entropy model. Without loss of generality, our framework takes the colored point cloud data as input. Note that, other attributes, such as opacity and reflectance, can also be compressed with our framework. }

%In this work, we focus on the task of point cloud attribute compression on large-scale point cloud scans, and assume that the geometry of point clouds has been separately transmitted and only compress the point cloud attributes. We propose an attribute compression method by exploiting the initial coding based and inter channel based context with a learning-based entropy model. The framework of our method is shown in Fig. \ref{fig:method_overview}. For simplicity, we use the colored point cloud data as an example. Note that, other attributes, such as opacity and reflectance, can also be compressed with our framework.

\qy{Specifically, we first apply an efficient 3D Haar wavelet transform (\ieours RAHT) to decompose point cloud attributes into low-frequency and high-frequency coefficients. The resulting high-frequency coefficients are quantized and formulated as a sequence of symbols. Then, we propose a learning-based entropy model utilizing both initial coding-based context and inter-channel-based context to model the probability distribution of each symbol. In the entropy coding stage, the predicted probabilities are further fed into an arithmetic coder to produce the final attribute bitstream.}


%Specifically, we first apply an efficient 3D Haar wavelet transform (i.e, RAHT) to decompose point cloud attributes into low-frequency and high-frequency coefficients. The resulting high-frequency coefficients are quantized and formulated as a sequence of symbols. Then, we propose a learning-based entropy model utilizing both initial coding based context and inter channel based context to model the probability distribution of each symbol. In the entropy coding stage, the predicted probabilities are fed into an arithmetic coder to produce the final attribute bitstream.
 

\subsection{Initial Coding}\label{sec:Initial Coding}


%The initial coding methods including \cite{de2016compression, pavez2020region, souto2020predictive, pavez2021multi} have the ability to capture spatial redundancy of point cloud attributes through the frequency domain representation. We adopt Region Adaptive Hierarchical Transform (RAHT) \cite{de2016compression}, for initial coding due to ease of construction, and it is possible to integrate the improved version of RAHT into our framework for better performance. 

\qy{As mentioned in the literature review, the initial coding methods including \cite{de2016compression, pavez2020region, souto2020predictive, pavez2021multi} are capable of capturing spatial redundancy of point cloud attributes through the frequency domain representation. Here, we adopt Region Adaptive Hierarchical Transform (RAHT) \cite{de2016compression} for initial coding due to its simplicity and flexibility. Note that, it is possible to integrate the improved version of RAHT into our framework for better performance. }



\subsubsection{Region Adaptive Hierarchical Transform}\label{raht}




RAHT is a variant of Haar wavelet transform, which convert point cloud attributes to frequency-domain coefficients. This method first voxelizes raw point clouds, and then decomposes attributes to low- and high-frequency coefficients through combining points from individual voxels to the entire voxel space. Here, we briefly revisit the RAHT \cite{de2016compression} through a 2D toy example.





Fig. \ref{fig:method_raht} shows the 2D example of RAHT. Only two dimensions, $x$ and $y$, are considered in this case. In Fig. \ref{fig:method_raht}(a), $l_{i}$ and $h_{i}$ denote low- and high-frequency coefficients, respectively. In the first block of Fig. \ref{fig:method_raht}(a), voxels filled with $l_{i}$ are occupied and should be transformed. We apply transform along the $x$ dimension first and then the $y$ dimension. In the encoding stage, at the first depth level, $l_{2}$ and $l_{3}$ are transformed to $l_{4}$ and $h_{1}$, and $l_{1}$ are transmitted to the next depth level directly due to lack of neighbor along $x$ dimension. In the second depth level, $l_{1}$ and $l_{4}$ are transformed to $l_{5}$ and $h_{2}$ along $y$ dimension. During decoding, the DC coefficient $l_{5}$ and all high-frequency coefficients $h_{1}$ and $h_{2}$ are required to restore low-frequency coefficients level by level. Thus, only these coefficients are quantized and transmitted as symbols.






% Fig. \ref{fig:method_raht} shows the 2D example of RAHT for encoding. Only two dimensions, $x$ and $y$, are considered in this case. In Fig. \ref{fig:method_raht}(a), $l_{i}$ and $h_{i}$ denote low- and high-frequency coefficients respectively. In the first block of Fig. \ref{fig:method_raht}(a), voxels filled with $l_{i}$ are occupied and should be transformed. We apply transform along the $x$ dimension first and then the $y$ dimension. At the first depth level, along the $x$ dimension, only $l_{6}$ and $l_{7}$ are transformed to $l_{8}$ and $h_{1}$, and other low-frequency coefficients are transmitted to the next depth level directly. Then, the pairs $(l_{3}, l_{4})$ and $(l_{5}, l_{6})$ are further transformed separately along the $y$ dimension. Transform is further conducted at the following depth level. Note that the decoding of RAHT is the inverse of the encoding process, so only the DC coefficient $l_{13}$ and all high-frequency coefficients $h_{i}$ are quantized and transmitted in order to recover low-frequency coefficients through the inverse of transform progressively.



For 3D point clouds, RAHT transforms attributes to low- and high-frequency coefficients along three dimensions repeatedly (\egours along the $x$ axis first, then the $y$ axis and the $z$ axis until merging all subspaces to the entire 3D space). The details about transforming from two low-frequency coefficients to low- and high-frequency coefficients can be found in \cite{de2016compression}.





% \qy{For 3D point clouds, RAHT sequentially transforms signals (\ieours, the attributes of nodes) to low- and high-frequency coefficients at each depth level along three dimensions (\egours, along the $x$ axis first, then the $y$ axis, and finally the $z$ axis). The details about transforming from two low-frequency coefficients to low- and high-frequency coefficients can be found in \cite{de2016compression}.}







% For point cloud data, RAHT sequentially transforms signals (i.e., the attributes of nodes) to low-fequency and high-frequency coefficients at each depth level along three dimensions (e.g., along the $x$ axis first, then the $y$ axis, and finally the $z$ axis). The low-frequency coefficient is passed to the next depth level if the node has no neighbor, and the transform is adopted when a neighbor exists using the following equation:
% \begin{equation}
% \left[\begin{array}{l}
% l_{d+1, x, y, z} \\
% h_{d+1, x, y, z}
% \end{array}\right]=\mathbf{T}_{w_{1}, w_{2}}\left[\begin{array}{c}
% l_{d, 2 x, y, z} \\
% l_{d, 2 x+1, y, z}
% \end{array}\right]\label{con:raht},
% \end{equation}
% where $l_{d, 2 x, y, z}$ and $l_{d, 2 x+1, y, z}$ are low-frequency coefficients of two neighboring nodes along the $x$ dimension, and $l_{d+1, x, y, z}$ and $h_{d+1, x, y, z}$ are the decomposed low-frequency and  high-frequency coefficients.Here, $\mathbf{T}_{w_{1}, w_{2}}$ is defined as
% \begin{equation}
% \mathbf{T}_{w_{1}, w_{2}}=\frac{1}{\sqrt{w_{1}+w_{2}}}\left[\begin{array}{cc}
% \sqrt{w_{1}} & \sqrt{w_{2}} \\
% -\sqrt{w_{2}} & \sqrt{w_{1}}
% \end{array}\right],
% \end{equation}
% where $w_{1}$ and $w_{2}$ are the weights (i.e., the number of leaf nodes) of $l_{d, 2x, y, z}$ and $l_{d, 2x+1, y, z}$, respectively. 

\subsubsection{RAHT Tree}\label{sec:raht_tree}


%Similar to octree initial coding for geometry compression \cite{huang2020octsqueeze, que2021voxelcontext, biswas2020muscle}, we are able to model RAHT with a tree structure for context feature extraction. In Figure \ref{fig:method_raht}(b), we construct a RAHT tree of the 2D toy example for better illustration. In the RAHT tree, leaf nodes represent original voxelized points and internal nodes represent the corresponding subspace. The position of a tree node is the center of the corresponding subspace. As shown in Figure \ref{fig:method_raht}(b), the low-frequency coefficient of a RAHT tree node is passed to its parent node if it has no neighbor along the transform direction (i.e. x or y for this 2D example), otherwise low- and high-frequency coefficients are generated for its parent node. We denote the parent node only containing low-frequency coefficients, as a low-frequency node (i.e. green nodes in Figure \ref{fig:method_raht}(b)), and other nodes containing both low- and high-frequency coefficients as high-frequency nodes (i.e. yellow nodes in Figure \ref{fig:method_raht}(b)).


\qy{Similar to octree initial coding for geometry compression \cite{huang2020octsqueeze, que2021voxelcontext, biswas2020muscle}, the RAHT can be also modeled with a tree structure for context feature extraction. Here, we show a constructed RAHT tree of the 2D toy example in Fig. \ref{fig:method_raht}(b). In the RAHT tree, leaf nodes represent original voxelized points and internal nodes represent the corresponding subspace. The position of a tree node is the center of the corresponding subspace. In particular, the low-frequency coefficient of a RAHT tree node is passed to its parent node if it has no neighbor along the transform direction (\ieours $x$ or $y$ for this 2D example), otherwise low- and high-frequency coefficients are generated for its parent node. 
We denote the parent node only containing low-frequency coefficients, as a low-frequency node (\ieours green nodes in Fig. \ref{fig:method_raht}(b)), and other nodes containing both low- and high-frequency coefficients as high-frequency nodes (\ieours yellow nodes in Fig. \ref{fig:method_raht}(b)).
}


\subsubsection{Serialization}\label{Serialization}

In order to utilize the initial coding-based context (\ieours low-frequency coefficients) in Section \ref{Initial Coding based Context Module}, we serialize the quantized high-frequency coefficients with a breadth-first traversal. At each depth level, we transmit the coefficients of different channels separately to explore the inter-channel correlation in Section \ref{Inter Channel based Context Module}. Following \cite{de2016compression}, uniform quantization is adopted and the only distortion comes from the quantization step. During decoding of the high-frequency coefficients, the mentioned context information is all accessible to our entropy model. For the DC coefficient, we transmit it directly. 






\subsection{Our Deep Entropy Model}

%According to the information theory \cite{shannon1948mathematical}, given the actual distribution of the transmitted high-frequency coefficients $\mathcal{R}$, a lower bound of bit-rate can be achieved by entropy coding. Unfortunately, the actual distribution $p(\mathcal{R})$ is unavailable in most cases. Therefore, we first formulate the estimated probability distribution $q(\mathcal{R})$ with initial coding information and inter channel correlation, and then adopt a deep neural network to approximate $q(\mathcal{R})$ with $p(\mathcal{R})$ by the cross-entropy.

\qy{According to the information theory \cite{shannon1948mathematical}, given the actual distribution of the transmitted high-frequency coefficients $\mathcal{R}$, a lower bound of bitrate can be achieved by entropy coding. However, the actual distribution $p(\mathcal{R})$ is usually unavailable in practice. Therefore, we first formulate the estimated probability distribution $q(\mathcal{R})$ with initial coding information and inter-channel correlation, and then adopt a deep neural network to approximate $q(\mathcal{R})$ with $p(\mathcal{R})$ \TBD{by the cross-entropy.}}




\subsubsection{Formulation}

%Considering both the number of attribute channels $n$ and points $m$, we denote high-frequency coefficients as $\mathcal{R}=\left\{\mathcal{R}^{(1)}, \ldots, \mathcal{R}^{(n)}\right\}$ and $\mathcal{R}^{(i)}=\left\{r_{1}^{(i)}, \ldots, r_{m}^{(i)}\right\}$. We first factorize $q(\mathcal{R})$ into a product of conditional probabilities taking account of the inter channel correlation as follows:

\qy{For 3D point clouds with $m$ points and $n$ attribute channels, the high-frequency coefficients are denoted as $\mathcal{R}=\left\{\mathcal{R}^{(1)}, \ldots, \mathcal{R}^{(n)}\right\}$ and $\mathcal{R}^{(i)}=\left\{r_{1}^{(i)}, \ldots, r_{m}^{(i)}\right\}$. By taking account of the inter channel correlation, we first factorize $q(\mathcal{R})$ into a product of conditional probabilities as follows:}


\begin{equation}
q(\mathcal{R})=\prod_{i} q\left(\mathcal{R}^{(i)} \mid \mathcal{R}^{(i-1)}, \ldots, \mathcal{R}^{(1)}\right),
\end{equation}
\qy{Here, the probability distribution of $\mathcal{R}^{(i)}$ is assumed to be depended on previous encoded sequences $\left\{\mathcal{R}^{(1)}, \ldots, \mathcal{R}^{(i-1)}\right\}$. It is noticed that the probability distribution $q(\mathcal{R})$ also depends on the information from the initial coding stage, hence we further factorize $q(\mathcal{R}^{(i)})$ with initial coding based context $\mathbf{I}_j$:
}
%We assume that the probability distribution of $\mathcal{R}^{(i)}$ depends on previous encoded sequences $\left\{\mathcal{R}^{(1)}, \ldots, \mathcal{R}^{(i-1)}\right\}$. 
%We observe that the probability distribution $q(\mathcal{R})$ also depends on the information from the initial coding stage, thus we further factorize $q(\mathcal{R}^{(i)})$ with initial coding based context $\mathbf{I}_j$:
\begin{equation}
q(\mathcal{R}^{(i)})=\prod_{j} q\left(r_{j}^{(i)} \mid \mathbf{I}_j, \mathcal{R}^{(i-1)}, \ldots, \mathcal{R}^{(1)}\right),
\end{equation}

\qy{Then, the estimated probability distribution $q\left(\cdot \mid \mathbf{I}_j, \mathcal{R}^{(i-1)}, \ldots, \mathcal{R}^{(1)}\right)$ can be modeled with a deep neural network. In particular, the network is mainly composed of initial coding based context module, inter channel based context module with a probability density model \cite{balle2018variational}.}

%Then, we model $q\left(\cdot \mid \mathbf{I}_j, \mathcal{R}^{(i-1)}, \ldots, \mathcal{R}^{(1)}\right)$ with a deep neural network. The network includes initial coding based context module in Section \ref{Initial Coding based Context Module} and inter channel based context module in Section \ref{Inter Channel based Context Module} with a probability density model \cite{balle2018variational}.

\subsubsection{Initial Coding based Context Module}\label{Initial Coding based Context Module}

%As mentioned in Section \ref{sec:Initial Coding}, we adopt RAHT for initial coding and represent the process of RAHT with a tree structure. In this section, we utilize the context information hidden in the initial coding stage through extracting context feature from both low- and high-frequency nodes denoted in Section \ref{sec:raht_tree}, and propose our initial coding based context module.

\qy{As mentioned in Section \ref{sec:Initial Coding}, we adopt RAHT for initial coding and represent the process of RAHT with a tree structure. Here, we exploit the contextual information hidden in the initial coding stage by extracting context features from both low- and high-frequency nodes, and propose our initial coding-based context module.}

\qy{\textbf{Learning context from high-frequency nodes.} We first start to process the information of high-frequency nodes. As mentioned in Section \ref{Serialization}, all high-frequency coefficients are quantized and transmitted as symbols in our framework. In light of the strong correlation between the high-frequency coefficients and the corresponding nodes, our initial coding-based context module follows \cite{huang2020octsqueeze} to extract the context feature $\mathbf{h}_j$ from each high-frequency node. In particular, we adopt a MultiLayer Perceptron (MLP) instead of an autoregressive model used in \cite{huang2020octsqueeze}, since the context information of a RAHT tree node is often redundant with that of its parent.  For a given high-frequency node, the context information contains the depth level, the weight (\textit{i.e.}, the number of child nodes), the low-frequency coefficient, and the attributes. Note that, all information is available during the progressive decoding stage. \TBD{(to do: more details list here or appendix? the low-frequency coefficient and the attributes are reconstructed during decoding). }
}


%We first include the information of high-frequency nodes into the initial coding based context feature. In Section \ref{Serialization}, all high-frequency coefficients are quantized and transmitted as symbols. We observe that there is a strong correlation between the high-frequency coefficients and the corresponding nodes. Thus, our initial coding based context module extracts the context feature $\mathbf{h}_j$ from each high-frequency node inspired by \cite{huang2020octsqueeze}. For a given high-frequency node, the context information contains the depth level, the weight (i.e., the number of child nodes), the low-frequency coefficient and the attributes. Note that all information is available during progressive decoding stage. (to do: more details list here or appendix? the low-frequency coefficient and the attributes is reconstructed during decoding). Distinct from \cite{huang2020octsqueeze}, we adopt a MultiLayer Perceptron (MLP) instead of an autoregressive model here because we observe that the context information of a RAHT tree node is redundant with that of its parent.

\qy{\textbf{Learning context from low-frequency nodes.} We further fuse the information of low-frequency nodes and high-frequency ones, and aggregate it into the initial coding-based context feature. Although low-frequency nodes do not interact directly with high-frequency coefficients in the initial coding stage, there remains a massive quantity of context information hidden in these nodes. Similarly, we also extract the context information that exists in low-frequency nodes, especially the depth level, the weight, the low-frequency coefficient, and the attributes. Here, we choose SparseConv \cite{4dMinkpwski, tang2020searching} to process RAHT tree nodes for efficiency. The detailed architecture is shown in  Fig. \ref{fig:method_sparse_conv_net}. In particular, \TBD{we perform 3D sparse convolutions at each depth level, and take both locations of low- and high-frequency nodes as input points and their context information mentioned above as input features. } With the progressive sparse convolution and downsampling, the context information of low-frequency nodes is fused with that of high-frequency nodes and diffused into multi-scale feature volumes. For each high-frequency node, we interpolate the latent feature from multi-scale feature spaces at their 3D location, and then concatenate them into a final latent feature $\mathbf{l}_j$.}


%\textbf{Information from Low-frequency Nodes.} We further fuse the information of low-frequency nodes and high-frequency ones, and aggregate it into the initial coding based context feature. Although low-frequency nodes do not interact directly with high-frequency coefficients in the initial coding stage, there remains a massive quantity of context information hidden in these nodes. As same as high-frequency nodes, low-frequency nodes also contain information including the depth level, the weight, the low-frequency coefficient and the attributes. Thus, our initial coding based context module further extracts the context information from them. For efficient feature extraction, we choose sparseconv \cite{4dMinkpwski, tang2020searching} to process RAHT tree nodes. Figure \ref{fig:method_sparse_conv_net} shows our sparseconv-based network architecture. Specifically, at each depth level, we utilizes 3D sparse convolutions, and take both locations of low- and high-frequency nodes as input points and their context information mentioned above as input features. With the sparse convolution and downsampling, the context information of low-frequency nodes is fused with that of high-frequency ones and diffused into multi-scale feature volumes. For each high-frequency node, we interpolate the latent feature from multi-scale feature spaces at their 3D location, and then concatenate them into a final latent feature $\mathbf{l}_j$.

We concatenate the context feature $\mathbf{h}_j$ and $\mathbf{l}_j$, and feed it into a MLP to obtain the initial coding based context $\mathbf{I}_j$ as follows:

\begin{equation}
\mathbf{I}_j=\mathrm{MLP}([\mathbf{h}_j, \mathbf{l}_j]).
\end{equation}





\subsubsection{Inter Channel based Context Module}\label{Inter Channel based Context Module}

In most cases, point cloud data contains multiple attribute channels (\textit{e.g.}, color, normal) and there is significant information redundancy between each channel. Thus, we propose our inter channel based context module to exploit the strong inter channel correlation.



\textbf{Inter Channel Coefficient Dependence.} For an uncompressed coefficient $ r_{j}^{(i)}$, our inter channel based context module first incorporates the previous encoded coefficients $\left\{r_{j}^{(1)}, \ldots, r_{j}^{(i-1)}\right\}$ to explore the inter channel coefficient dependence. Specifically, we adopt the previous encoded coefficients as context information and feed them into a MLP to extract the context feature $\mathbf{c}_{j}^{(i)}$ as follows:

\begin{equation}
\mathbf{c}_{j}^{(i)}=\mathrm{MLP}([r_{j}^{(1)}, \ldots, r_{j}^{(i-1)}]).
\end{equation}
Here, we simply concatenate all previous encoded coefficients as the input of the MLP.




\textbf{Inter Channel Spatial Dependence.} We further aggregate the encoded coefficient information utilizing the spatial relation between tree nodes to benefit the probability estimation. A key observation is that coefficients of other tree nodes are also helpful to predict the coefficient of a certain node. Specifically, we incorporate all high-frequency nodes at the same depth level  and utilize their encoded coefficients through 3D sparse convolution. Note that only high-frequency nodes are considered in this part because they contain encoded coefficients and others do not. The inter channel spatial context feature $\mathbf{s}_j^{(i)}$ is obtained through the similar network architecture as Fig. \ref{fig:method_sparse_conv_net} with locations of high-frequency nodes as input points and previous encoded coefficients as input features. For the model consistency, we set the context feature of the first channel $\mathbf{c}_{j}^{(1)}$ and $\mathbf{s}_j^{(1)}$ as all zeros features. 


Similar to the feature aggregation of initial coding based context feature, we concatenate $\mathbf{c}_{j}^{(i)}$ and $\mathbf{s}_j^{(i)}$, and feed it into a MLP to obtain the inter channel based context $\mathbf{C}_j^{(i)}$. Thus, we can finally model $q\left(r_{j}^{(i)} \mid \mathbf{I}_j, \mathcal{R}^{(i-1)}, \ldots, \mathcal{R}^{(1)}\right)$ as $q(r_{j}^{(i)} \mid \mathbf{I}_j, \mathbf{C}_j^{(i)})$.





\subsubsection{Probability Estimation}


We aggregate the initial coding based context $\mathbf{I}_j$, the inter channel based context feature $\mathbf{C}_j^{(i)}$ through a MLP to obtain the final latent feature. This latent feature is further adopted to generate learnable parameters for a fully factorized density model \cite{balle2018variational}, which is able to model the probability distribution $q\left(r_{j}^{(i)} \mid \mathbf{I}_j, \mathcal{R}^{(i-1)}, \ldots, \mathcal{R}^{(1)}\right)$. (architecture details here or appendi?)



% necessary or not? + run time analysis 
\subsection{Entropy Coding}

At the encoding stage, we adopt an arithmetic coder to obtain the final attribute bitstream. We compress the quantized high-frequency coefficients from root to leaves of the RAHT tree. At each depth level, we compress coefficients of different channel separately with the estimated probability distribution from our deep entropy model. The DC coefficient is transmitted directly.

At the decoding stage, the same entropy model and the arithmetic coder are used for decompression. We decode the high-frequency coefficients from root to leaves. With the inverse of RAHT, low-frequency coefficients are recovered level by level. At each depth level, we decode coefficients of different channel in a progressive manner. Thus, we runs at $O(D \times N)$ GPU passes for our entropy model per point cloud, where $D$ is the maximum depth level of RAHT tree and $N$ is the number of attributes. 

% $O(D \times n)$
% $O(D \cdot n)$

\subsection{Learning}

%At training time, we train our deep entropy model with cross-entropy loss:
\qy{During training, we adopt the cross-entropy loss for the  deep entropy model:}
% \begin{equation}
% \ell=-\sum_{i}\sum_{j} \log q\left(r_{j}^{(i)} \mid \mathbf{I}_j, \mathcal{R}^{(i-1)}, \ldots, \mathcal{R}^{(1)}\right).
% \end{equation}
\begin{equation}
\ell=-\sum_{i}\sum_{j} \log q(r_{j}^{(i)} \mid \mathbf{I}_j, \mathbf{C}_j^{(i)}).
\end{equation}
\qy{To reduce the bitrate of the final attribute bitstream, we approximate the estimated distribution $q(\mathcal{R})$ with the actual distribution $p(\mathcal{R})$  by minimizing the cross-entropy loss.}
%We approximate the estimated distribution $q(\mathcal{R})$ with the actual distribution $p(\mathcal{R})$ by minimizing the cross-entropy loss to reduce the bitrate of the final attribute bitstream.









==> chapters/030_method_v0.tex <==

% \begin{figure}[t]
% 	\begin{center}
% 		\includegraphics[width=1.0\linewidth]{Figures/method/method_overview.png}
% 	\end{center}
%     \caption{}
% 	\label{fig:method_overview}
% \end{figure}




\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/method/method_raht.pdf}
	\end{center}
    \caption{An illustration of RAHT and RAHT binary tree. (a) A 2D example of RAHT, (b) a RAHT binary tree.}
	\label{fig:method_raht}
\end{figure*}











% Overview
\subsection{Overview}

%\TBD{In this work, we focus on the task of point cloud attribute compression on large-scale point cloud scans.} 
\gary{In this work, we mainly focus on point cloud attribute compression, i.e., we assume that the geometry of point clouds has been separately compressed. The framework of our wavelet-based deep compression method is shown in Fig. \ref{fig:method_overview}. For simplicity, we use the color of points as an example attribute for compression.  
Note that, other attributes, such as opacity and reflectance, can also be compressed with our framework.}


%Assuming that point cloud geometry (positions of points) has been separately encoded and transmitted, the challenge of this task is to preserve attribute reconstruction quality as well as reducing the attribute bitstream size. In order to deal with this problem, we propose a wavelet-based deep compression method. Figure \ref{fig:method_overview} shows the overall framework of our method. For simplicity, we take colored point cloud data as an example. Note that this framework can be simply extended to point cloud with other attributes, such as opacity and reflectance.

\gary{Specifically, we firstly apply an efficient 3D wavelet transform (i.e, RAHT) to decompose point cloud attributes into low-frequency and high-frequency coefficients based on the given point cloud \TBD{geometry}. The resulting wavelet coefficients are quantized and formulated as uncompressed symbols. Then, we propose a learning-based entropy model to estimate the Probability Mass Function (PMF) of these symbols. During entropy modeling, RAHT-node context and RAHT-geometry context are extracted from the RAHT binary tree and the point cloud geometry to generate RAHT context features. An inter-channel prediction module is additionally included to reduce the redundancy within multiple channels. Finally, the predicted probabilities are fed into an arithmetic \TBD{en}coder to produce the final attribute bitstream.}



% \begin{figure}[t]
% 	\begin{center}
% 		\includegraphics[width=1.0\linewidth]{Figures/method/method_octree.png}
% 	\end{center}
%     \caption{}
% 	\label{fig:method_octree}
% \end{figure}









% \begin{figure}[t]
% 	\begin{center}
% 		\includegraphics[width=1.0\linewidth]{Figures/method/method_various_context.png}
% 	\end{center}
%     \caption{}
% 	\label{fig:method_various_context}
% \end{figure}

% \begin{figure}[t]
% 	\begin{center}
% 		\includegraphics[width=1.0\linewidth]{Figures/method/method_geom_comparsion.png}
% 	\end{center}
%     \caption{}
% 	\label{fig:method_geom_comparsion}
% \end{figure}






% Octree Construction and Region Adaptive Hierarchical Transform
\subsection{Region Adaptive Hierarchical Transform}\label{section:raht}
%这部分需要重点修改

% The qualitative result shown in Figure \ref{fig:teaser} indicates that the existing deep image compression methods are not able to extend to point cloud attribute compression directly due to the failure of attribute reconstruction. In other words, the main challenge of point cloud attribute compression is how to preserve reconstruction quality. Transform-based methods [] adopt signal processing techniques to transform point cloud attribute to corresponding coefficients 

\gary{RAHT is used to efficiently extract point cloud representation based on an octree.}

%The qualitative result shown in Figure \ref{fig:teaser} indicates that the existing point cloud learning methods fail in attribute reconstruction. In contrast, traditional signal processing techniques [] show their strong ability of representing point cloud data. We choose to use region adaptive hierarchical transform (RAHT) due to its efficiency and ability of representation. Because RAHT is based on an octree, we briefly introduce the octree structure first and then RAHT.

\gary{An octree is constructed by recursively partitioning a 3D space into 8 equal cubes  until the maximum depth. For each level of the octree, non-empty cubes are stored and represented as an octree node. RAHT is a variation of 3D wavelet transform based on an octree. \TBD{Following the octree scan backwards}, RAHT transforms signals (i.e., the attributes of nodes) to low-fequency and high-frequency coefficients at each depth level. Similar to 2D wavelet transform, RAHT sequentially decomposes signals along all dimensions (e.g., along the $x$ axis first, then the $y$ axis, and finally the $z$ axis) with the following transform:
%comments:直接上来就是公式，过渡太生硬，不容易让人懂。考虑把下文的例子挪到上面来。结合例子来介绍。
\begin{equation}
\left[\begin{array}{l}
l_{d+1, x, y, z} \\
h_{d+1, x, y, z}
\end{array}\right]=\mathbf{T}_{w_{1}, w_{2}}\left[\begin{array}{c}
l_{d, 2 x, y, z} \\
l_{d, 2 x+1, y, z}
\end{array}\right]\label{con:raht},
\end{equation}
where $l_{d, 2 x, y, z}$ and $l_{d, 2 x+1, y, z}$ are low-frequency coefficients of two neighboring nodes along the $x$ dimension, and $l_{d+1, x, y, z}$ and $h_{d+1, x, y, z}$ are the decomposed low-frequency and  high-frequency coefficients.}

\gary{Here, $\mathbf{T}_{w_{1}}$ is defined as
\begin{equation}
\mathbf{T}_{w_{1}, w_{2}}=\frac{1}{\sqrt{w_{1}+w_{2}}}\left[\begin{array}{cc}
\sqrt{w_{1}} & \sqrt{w_{2}} \\
-\sqrt{w_{2}} & \sqrt{w_{1}}
\end{array}\right],
\end{equation}
where $w_{1}$ and $w_{2}$ are the weights (i.e., the number of leaf nodes) of $l_{d, 2x, y, z}$ and $l_{d, 2x+1, y, z}$, respectively. Low-frequency coefficients are directly passed to the next level if the node does not have a neighbor. Finally, high-frequency coefficients are quantized and transmitted as symbols. In this work, we construct a RAHT binary tree (as shown in Fig. \ref{fig:method_raht}(b)) instead of octree for feature extraction (more in Section \ref{section:raht_context}).}

\gary{We take a 2D example for further illustration, as shown in Fig. \ref{fig:method_raht}. $l_{d, x, y}$ and $h_{d, x, y}$ denote low- and high-frequency coefficients at depth $d$ and position $(x, y)$. We apply RAHT along the $x$ dimension and then the $y$ dimension. At the first depth level, along the $x$ dimension, only $l_{0, 2, 3}$ and $l_{0, 3, 3}$ are transformed to $l_{1, 1, 3}$ and $h_{1, 1, 3}$ according to Eq. \ref{con:raht}. At the next level, the pairs $(l_{1, 0, 2}, l_{1, 0, 3})$ and $(l_{1, 1, 2}, l_{1, 1, 3})$ are further transformed. RAHT is progressively conducted at each depth level, the DC coefficient ($l_{4, 0, 0}$) and all high-frequency coefficients $h_{d, x, y}$ are quantized and transmitted. During decoding, low-frequency coefficients can be regenerated using the decompressed high-frequency coefficients according to the inverse of Eq. \ref{con:raht}. In this stage, context information is also available for decoding.}


% $\left[\begin{array}{l}g_{l-1, x, y, z} \\ h_{l-1, x, y, z}\end{array}\right]=\mathbf{T}_{w_{1} w_{2}}\left[\begin{array}{c}g_{l, 2 x, y, z} \\ g_{l, 2 x+1, y, z}\end{array}\right]$

% $\mathbf{T}_{w_{1} w_{2}}=\frac{1}{\sqrt{w_{1}+w_{2}}}\left[\begin{array}{cc}\sqrt{w_{1}} & \sqrt{w_{2}} \\ -\sqrt{w_{2}} & \sqrt{w_{1}}\end{array}\right]$


% Low-frequency coefficients are passed along to the next levle and high-frequency coefficients are ready for transmission.







% Various Context
\subsection{RAHT Context}\label{section:raht_context}
%%comments：这一段需要重写，主要写清楚为什么需要RAHT Context？主要想解决什么问题？把motivation讲清楚。这里不需要将前人的工作怎么样，主要讲你为什么要这么做，怎么做，可能有什么效果。

%Prior works of point cloud attribute compression [] transform point cloud attributes to coefficients and encode the coefficients to bitstream separately, resulting in the inefficient utilization of data priors of the coefficients and the raw data. However, most existing learning-based methods [] focus on point cloud geometry compression, which is quite different from attribute compression. There are two major differences: 1) the distinct initial encoding methods (octree coding or singal transform coding), and 2) point cloud geometry has or has not been transmitted. Considering these factors, we develop RAHT context, including RAHT-Node context and RAHT-Geometry context, for our deep entropy model.


\subsubsection{RAHT-Node Context} 
\gary{Once a RAHT binary tree for context extraction is constructed in the initial RAHT encoding step, the context information is available during decoding. For each node, the RAHT-node context includes the depth level of the RAHT binary tree, the weight (i.e., the number of  child nodes), the 3D location of the node, the low-frequency coefficient reconstructed at the node during decoding, and the  attribute reconstructed at the node during decoding (through inverse of RAHT according to Eq. \ref{con:raht} ).}
%comments: 不清楚为什么这里需要用到decoding的信息？这里不是还在编码的阶段吗？

%Here, `depth' is the depth level of the RAHT binary tree, 'weight' is the number of the child nodes, 'location' is the node's location in 3D space, and 'reconstructed low-frequency coefficient' and 'reconstructed attribute' are node's reconstructed low-frequency coefficient and attribute through inverse of RAHT according to the Equation \ref{con:raht} during decoding time.

%As illustrated in Section \ref{section:raht}, we constuct a RAHT binary tree for context extraction in initial RAHT encoding step. Note that context information should be available during decoding time. For each node, the RAHT-node context includes depth, weight, location, reconstructed low-frequency coefficient and reconstructed attribute. Specifically, 'depth' is the depth level of the RAHT binary tree, 'weight' is the number of the child nodes, 'location' is the node's location in 3D space, and 'reconstructed low-frequency coefficient' and 'reconstructed attribute' are node's reconstructed low-frequency coefficient and attribute through inverse of RAHT according to the Equation \ref{con:raht} during decoding time.


\subsubsection{RAHT-Geometry Context} 
\gary{Since point cloud attribute compression assumes that point cloud geometry has been transmitted, geometry context is available for both attribute encoding and decoding. %Compared with previous works [] only using node's location and nearby voxels as context, 
In this paper, we use multi-scale geometry information through sparse convolution [] and develop RAHT-geometry context by combining both RAHT-Node context and geometry context. More specifically, for each depth level, \TBD{we extract latent feature maps using sparse convolution with location of nodes as the input point cloud and RAHT-Node context as the input point cloud feature.} Then, we use trilinear interpolation to obtain multi-level latent feature of each node and concatenate these features to produce RAHT-geometry context, as shown in Fig. \ref{fig:method_sparse_conv_net}. These features are then fused with 3 Multi-Layer Perceptrons (MLPs) for our deep entropy model.}


\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/method/method_sparse_conv_net.pdf}
	\end{center}
    \caption{RAHT-geometry context learning with SparseConvNet.}
	\label{fig:method_sparse_conv_net}
\end{figure}

%After extraction of RAHT-Node context and RAHT-Geometry context, we concatenate these context features and use 3 multi-layer perceptrons (MLPs) to fuse these features for our deep entropy model.



% Inter Channel Prediction
\subsection{Inter-channel Prediction}\label{section:inter_channel_prediction}

\gary{Since there is considerable information redundancy within multiple channels, we further propose an inter-channel prediction module to improve compression performance. %Taking RGB color mode as an example, we can better predict the blue channel if the red and green channels are known. 
We predict and encode symbols in a progressive manner for each channel. Given the symbols $s_{i,0}$, $s_{i,1}$ and $s_{i,2}$ of 3 channels  to be encoded at node $i$ and the RAHT context $\mathbf{R}$, the fused context feature $\mathbf{f_{i,0}}$, $\mathbf{f_{i,1}}$ and $\mathbf{f_{i,j+2}}$ are determined as:
\begin{equation}
\begin{aligned}
\mathbf{f}_{i,0}&=\mathbf{R}, \\
\mathbf{f}_{i,1}&=\mathrm{MLP}\left(\mathbf{R},s_{i,0} \right), \\
\mathbf{f}_{i,2}&=\mathrm{MLP}\left(\mathbf{R},s_{i,0}, s_{i,1}\right).
\end{aligned}
\end{equation}
}



% \begin{equation}
% q(\mathbf{x})=\prod_{i} q_{i}\left(x_{i} \mid \mathbf{x}_{\mathbf{a n}(i)}, \mathbf{c}_{i} ; \mathbf{w}\right)
% \end{equation}

% $q(\mathbf{x})=\prod_{i} q_{i}\left(x_{i} \mid \mathbf{x}_{\mathbf{a n}(i)}, \mathbf{c}_{i} ; \mathbf{w}\right)$


% Our Deep Entropy Model
\subsection{Deep Entropy Model}

%\smallskip\noindent
\subsubsection{Formulation} 
\gary{Given a colored point cloud, we quantize the high-frequency coefficients in 3 channels as the symbols. %\TBD{For node $i$, $\mathbf{s_{i}}$ and $\mathbf{f_{i}}$ are the corresponding symbols and context feature. $\mathbf{s_{i}=\left[s_{i,0}, s_{i,1}, s_{i,2}\right]}$ are symbols for 3 channels.}
%and $\mathbf{s}=\left[s_{0}, \ldots, s_{i}, \ldots\right]$ is the sequence of symbols.
We further compress these symbols to an attribute bitstream with entropy coding. According to the information theory, given the actual distribution of transmitted symbols, a lower bound of bit-rate can be achieved by entropy coding. 
Unfortunately, the actual distribution is unavailable in most cases. Therefore, we propose a wavelet-based deep entropy model to estimate the probability distribution of occupancy symbols.}
%Thus, prior works [] propose their own deep entropy model, adopting a deep neural network to estimate the probability distribution of occupancy symbols. However, these existing deep entropy models focus on the task of point cloud geometry compression and can not directly extend to other tasks, such as point cloud attribute compression. As described in Section \ref{section:raht_context}, we extract RAHT context and propose our wavelet-based deep entropy model. 
%对现有工作的评述不应该放在method部分。在method部分，只需要专注于介绍你的工作。可以把相应的评述整理一下，放到related work里


\gary{Considering the range of our symbols generated by RAHT, we follow [] to estimate the probability mass function $q(\mathbf{s})$ of symbols as follows,
% \prod_{i,j} ? 
\begin{equation}
q(\mathbf{s})=\prod_{i,j} q\left(s_{i,j} \mid \mathbf{f}_{i}\right)\label{con:pmf},
\end{equation}
where $\mathbf{f}_{i}$ is the fused context feature of node $i$ from the RAHT context and the inter-channel prediction module.}

\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/exp/exp_quant.pdf}
	\end{center}
    \caption{Results of different attribute compression methods on two benchmark datasets ScanNet \& Semantic KITTI.}
	\label{fig:exp_scannet}
\end{figure*}

\subsubsection{Network Architecture}
\gary{We adopt neural networks to formulate our deep entropy model as Eq. \ref{con:pmf}. As described in Sec. \ref{section:raht_context}, we extract RAHT-node context from the RAHT binary tree. We adopt 3 sparse convolution layers to obtain multi-level feature maps and then use trilinear interpolation to query the latent feature at the 3D location of the node. Then, a MLP is adopted to generate a 8-dimensional latent feature, which is our RAHT-geometry context. Next, we concatenate RAHT-node context feature and RAHT-Geometry context feature and use 3 MLPs to obtain the RAHT context feature. We further feed the transmitted symbols as contextual information into MLPs with RAHT context feature (as described in Sec. \ref{section:inter_channel_prediction}) to obtain the fused context feature. A fully factorized density model [] is constructed with the fused context feature as its parameters.}

% Training Strategy
\subsection{Training Strategy}
%comments:需要说明下为什么用这个loss来做训练？
\gary{At training time, we train our deep entropy model with the following loss function:
\begin{equation}
l=-\sum_{i}\sum_{j} \log q_{s_{i,j}}\left({s}_{i,j} \mid \mathbf{f}_{i}\right).
\end{equation}
where $q_{s_{i,j}}$ is the estimated probability distribution of symbol $s_{i,j}$ and ${f}_{i}$ is the context feature of node $i$.}



==> chapters/040_Experiments_v0.tex <==



\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/exp/exp_quant.pdf}
	\end{center}
    \caption{Results of different attribute compression methods on two benchmark datasets ScanNet \& Semantic KITTI.}
	\label{fig:exp_scannet}
\end{figure*}





\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/exp/scannet/exp_qual_scannet_skitti2.pdf}
	\end{center}
    \caption{Qualitative results of our and the comparison methods including Spconv AE, RAHT [] and G-PCC []. We visualize ScanNet scans with RGB colors and Semantic KITTI with intensity of reflectance. The first and the third row are the reconstruction results at relative low bitrates and the others are at high bitrates.}
	\label{fig:exp_qual_scannet}
\end{figure*}









% \begin{figure}[t]
% 	\begin{center}
% 		\includegraphics[width=1.0\linewidth]{Figures/exp/exp_ab.png}
% 	\end{center}
%     \caption{}
% 	\label{fig:exp_ab}
% \end{figure}




\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figures/exp/exp_scannet_seg.pdf}
	\end{center}
    \caption{Quantitative results. }
	\label{fig:scannet_seg}
\end{figure}





%comments:在这里补充一段话，介绍这一个section的总体安排
\subsection{Datasets}
\textbf{ScanNet:} 
\gary{We used ScanNet \cite{} to test the compression performance of our method on indoor 3D scans. ScanNet is a large-scale point cloud dataset containing 1513 indoor scans. Each scan contains over ten thousand colored points. Following the experimental setting of [], we used 1,201 point clouds for training and 312 point clouds for testing. Since point cloud color is useful for many 3D perception tasks, we further evaluate the performance of downstream tasks on this dataset.}

\textbf{Semantic KITTI:} 
\gary{We used SemanticKITTI \cite{} to test the performance of our method on outdoor LiDAR point clouds. The SemanticKITTI dataset contains 22 point cloud sequences. We take point cloud reflectance, a most common attribute captured by LiDAR sensors, as the attribute for compression. Following the default setting in \cite{}, we used 11 point sequences for training and the other 11 sequences for test.}

\subsection{Experimental Setting}
\textbf{Baselines.} 
\gary{We compare our method to two state-of-the-art hand-crafted point cloud compression methods (i.e., RAHT [] and RAGFT []) and the standard point cloud compression method (G-PCC) provided in MPEG. 
In G-PCC, adaptive quantization is used to quantize coefficients while 0-run length coding is used for entropy coding. RAGFT is a variant of RAHT with graph transform. We used uniform quantization and the  runlength Golomb-Rice coder for both RAHT and RAGFT. Besides, we also compare our method to a 3D auto-encoder based method (i.e., Spconv AE). We adopt MinkUNet [] to extract latent features and a probability density model [] as the deep entropy model. Attributes are reconstructed by the 3D auto-encoder during decoding.}

\textbf{Implementation Details.} 
\gary{We transmitted the geometry of point clouds without loss and converted attributes of point clouds from RGB to YUV color space for the ScanNet dataset. We constructed octrees of 9 levels and 12 levels, and RAHT binary trees of 27 levels and 36 levels for the ScanNet and SemanticKITTI datasets, respectively. 
High-frequency coefficients were uniform quantized and compressed with the estimated probability and the DC coefficient was transmitted separately. }

\gary{Our network was implemented in PyTorch and trained with one NVIDIA 1080TI GPU. We used the Adam optimizer with an initial learning rate of 0.01 for 20 epochs.}


\textbf{Evaluation Metrics.} 
\gary{Following [], we used peak signal-to-noise ratio of the luminance component ($\rm PSNR_y$ in dB) to evaluate the reconstruction quality on the ScanNet dataset. Since reflectance was considered as the attribute of points on the  Semantic KITTI dataset, we therefore 
used $\rm PSNR$ of reflectance to test the reconstruction quality on this dataset. Besides, we used Bits Per Point ($\rm BPP$) to evaluate the compression ratio.}


\subsection{Experiment Results}
%Results on scannet

\subsubsection{Results on the ScanNet Dataset}

\gary{The rate-distortion curves achieved by all methods on the ScanNet dataset are shown in Fig. \ref{fig:exp_scannet}. Our method achieves competitive compression performance to all other methods. \TBD{Due to failure in reconstruction}, the 3D auto-encoder based method (i.e., Spconv AE) achieves the worst compression performance.  Note that,  the same initial coding method was adopted by our method and RAHT []. However, our method achieves a much lower bitrate at the same reconstruction PSNR as compared to RAHT. Moreover, our method achieves  comparable performance to RAGFT and G-PCC at low bitrates, and significantly outperforms these methods at high bitrates. More specifically, the average BPP of our method is 8.86 and the corresponding $\rm PSNR_y$ is 53.03 dB. In contrast, the BPPs of G-PCC and RAGFT are 11.21 and 9.72, and their coresponding $\rm PSNR_y$ values are 51.89 dB and 53.01 dB, respectively.}

\gary{We also show the qualitative results on ScanNet in Fig. \ref{fig:exp_qual_scannet}. The first row and the second row show the reconstruction results at low and high bitrates, respectively. Our approach achieves the best reconstruction performance, especially at high bitrates. Note that, all other methods significantly outperform 3D auto-encoder based methods. That is because, the 3D auto-encoders are unable to preserve high-frequency information, leading to failures in the reconstruction of attribute details.}

\subsubsection{Results on the Semantic KITTI Dataset.}
\gary{The compression results achieved by different methods on the Semantic KITTI dataset are shown in Fig. \ref{fig:exp_scannet}. It can be observed that our method outperforms other methods by a large margin. It can be inferred that our learning based method works well on both dense and sparse point clouds, while the existing methods (including RAHT, RAGFT and G-PCC) are mainly developed for dense point clouds. From the qualitative results shown in Fig. \ref{fig:exp_qual_scannet}, it is also clear that our method achieves better performance than the state-of-the-art methods.}
%需要解释下为什么我们的方法对稀疏的点云上也能做的很好？在方法设计上，我们有什么样的特别考虑，使得其具有这样的性能。
%Considering that methods including RAHT, RAGFT and G-PCC are all developed on the dense point clouds similar to scans of ScanNet, our learning-based method outperforms all these methods on sparse lidar point cloud scans. We also observe that the qualitative results of our method are better compared with these methods as show in Figure \ref{fig:exp_qual_scannet}. 





%comparsion with gpcc

%\textbf{comparsion with gpcc}




\input{Tables/ablation}



\subsection{Ablation Study and Analysis}
\textbf{Effectiveness of Our Proposed Components. }
\textbf{depth}

\textbf{Computational Complexity }
ours 1.862718792, 1.847826022
gpcc 0.3586




\textbf{Experimental Results for the Downstream Tasks }



==> chapters/060_Discussions.tex <==
% \bo{Whilst the proposed \nickname{} achieves remarkable results in semantic segmentation with extremely weak supervision, it also has limitations. First, the assumption about the consistency of neighborhood semantics does not hold at the boundary areas with different semantics. Future works will further explore how to achieve more precise segmentation performance at boundaries. Second, our feature extractor is still limited to capture precise point features, more advanced encoding architecture will be used in future work. We believe this is the major reason why our \nickname{} still lags behind some state-of-the-art fully-supervised methods. 
% }

%as the generated pseudo-labels will inevitably have some errors, the erroneous supervision signal provided may degrade the segmentation performance in some respects. To this end, it would be interesting to further investigate how to best to learn from imprecise and noisy supervisory signals.


==> chapters/symbol_table.tex <==



% high freq coefficient R,r
% probability q,p
% initial coding based context I

% the context information h_j
% latent feature l_j

% Inter Channel Coefficient Dependenc c_j^i
% Inter Channel Spatial Aggregation s_j^i


1. rescale figure of quantative results
2. downstream task: delete segmentation, replace with flow estiamtion
3. add 'comparison with learning-based methods' in appendix
4. RAHT writing








==> chapters/test.tex <==

\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{Figures/exp/exp_downstream.pdf}
	
    \caption{Quantitative results}
	\label{fig:exp_qual_scannet}
\end{figure*}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{sample/Figures/040_Experiments/exp_downstream.pdf}
	
%     \caption{downstream tasks}
% 	\label{fig:exp_qual_scannet}
% \end{figure}

why not figure?

\begin{figure}[b]
	\begin{center}
	\includegraphics[width=1.0\linewidth]{Figures/exp/exp_downstream.pdf}
	\end{center}
    \caption{The quantitative results for two downstream tasks. 
    }
	\label{fig:scannet_seg}
\end{figure}


==> egbib_full.tex <==
@inproceedings{rao2010grasping,
  title={Grasping novel objects with depth segmentation},
  author={Rao, Deepak and Le, Quoc V and Phoka, Thanathorn and Quigley, Morgan and Sudsang, Attawith and Ng, Andrew Y},
  booktitle={2010 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={2578--2585},
  year={2010},

}

@inproceedings{valada2017adapnet,
  title={Adapnet: Adaptive semantic segmentation in adverse environmental conditions},
  author={Valada, Abhinav and Vertens, Johan and Dhall, Ankit and Burgard, Wolfram},
  booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={4644--4651},
  year={2017},

}

@inproceedings{Matterport3D,
  title={{Matterport3D}: Learning from {RGB-D} data in indoor environments},
  author={Chang, Angel and Dai, Angela and Funkhouser, Thomas and Halber, Maciej and Niebner, Matthias and Savva, Manolis and Song, Shuran and Zeng, Andy and Zhang, Yinda},
  booktitle={7th IEEE International Conference on 3D Vision, 3DV 2017},
  pages={667--676},
  year={2018},
}

@article{geiger2013vision,
  title={Vision meets robotics: The kitti dataset},
  author={Geiger, Andreas and Lenz, Philip and Stiller, Christoph and Urtasun, Raquel},
  journal={The International Journal of Robotics Research},
  volume={32},
  number={11},
  pages={1231--1237},
  year={2013},
}

@article{cornelis20083d,
  title={3{D} urban scene modeling integrating recognition and reconstruction},
  author={Cornelis, Nico and Leibe, Bastian and Cornelis, Kurt and Van Gool, Luc},
  journal={International Journal of Computer Vision},
  volume={78},
  number={2-3},
  pages={121--141},
  year={2008},
}

@article{austin2020architecting,
  title={Architecting smart city digital twins: combined semantic model and machine learning approach},
  author={Austin, Mark and Delgoshaei, Parastoo and Coelho, Maria and Heidarinejad, Mohammad},
  journal={Journal of Management in Engineering},
  volume={36},
  number={4},
  year={2020},
}

@article{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Advances in Neural Information Processing Systems},
  volume={25},
  pages={1097--1105},
  year={2012}
}

@inproceedings{long2015fcn,
  title={Fully convolutional networks for semantic segmentation},
  author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3431--3440},
  year={2015}
}

@inproceedings{girshick2015fast,
  title={Fast {R}-{CNN}},
  author={Girshick, Ross},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1440--1448},
  year={2015}
}

@article{Microsoft_kinect,
  title={Microsoft kinect sensor and its effect},
  author={Zhang, Zhengyou},
  journal={IEEE multimedia},
  volume={19},
  number={2},
  pages={4--10},
  year={2012},
}

@inproceedings{3d_shapenets,
  title={3{D} {ShapeNets}: A deep representation for volumetric shapes},
  author={Wu, Zhirong and Song, Shuran and Khosla, Aditya and Yu, Fisher and Zhang, Linguang and Tang, Xiaoou and Xiao, Jianxiong},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1912--1920},
  year={2015}
}


@article{chang2015shapenet,
  title={Shape{N}et: An information-rich 3{D} model repository},
  author={Chang, Angel X and Funkhouser, Thomas and Guibas, Leonidas and Hanrahan, Pat and Huang, Qixing and Li, Zimo and Savarese, Silvio and Savva, Manolis and Song, Shuran and Su, Hao and others},
  journal={arXiv preprint arXiv:1512.03012},
  year={2015}
}


@inproceedings{scenenn,
  title={Scene parsing through {ADE20K} dataset},
  author={Zhou, Bolei and Zhao, Hang and Puig, Xavier and Fidler, Sanja and Barriuso, Adela and Torralba, Antonio},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={633--641},
  year={2017}
}

@inproceedings{lang2019pointpillars,
  title={Pointpillars: Fast encoders for object detection from point clouds},
  author={Lang, Alex H and Vora, Sourabh and Caesar, Holger and Zhou, Lubing and Yang, Jiong and Beijbom, Oscar},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12697--12705},
  year={2019}
}

@article{ShapePartNet,
  title={A scalable active framework for region annotation in 3{D} shape collections},
  author={Yi, Li and Kim, Vladimir G and Ceylan, Duygu and Shen, I-Chao and Yan, Mengyan and Su, Hao and Lu, Cewu and Huang, Qixing and Sheffer, Alla and Guibas, Leonidas},
  journal={ACM Transactions on Graphics (TOG)},
  volume={35},
  number={6},
  pages={1--12},
  year={2016},
}

@inproceedings{mo2019partnet,
  title={{PartNet}: A large-scale benchmark for fine-grained and hierarchical part-level 3{D} object understanding},
  author={Mo, Kaichun and Zhu, Shilin and Chang, Angel X and Yi, Li and Tripathi, Subarna and Guibas, Leonidas J and Su, Hao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={909--918},
  year={2019}
}

@inproceedings{scanobjectnn,
  title={Revisiting point cloud classification: A new benchmark dataset and classification model on real-world data},
  author={Uy, Mikaela Angelina and Pham, Quang-Hieu and Hua, Binh-Son and Nguyen, Thanh and Yeung, Sai-Kit},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1588--1597},
  year={2019}
}

@inproceedings{NYU3D,
  title={Indoor segmentation and support inference from {RGBD} images},
  author={Silberman, Nathan and Hoiem, Derek and Kohli, Pushmeet and Fergus, Rob},
  booktitle={European conference on computer vision},
  pages={746--760},
  year={2012}
}

@inproceedings{sunrgbd,
  title={Sun {RGB-D}: A {RGB-D} scene understanding benchmark suite},
  author={Song, Shuran and Lichtenberg, Samuel P and Xiao, Jianxiong},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={567--576},
  year={2015}
}

@article{scenenetrgbd,
  title={{SceneNet RGB-D}: 5M photorealistic images of synthetic indoor trajectories with ground truth},
  author={McCormac, John and Handa, Ankur and Leutenegger, Stefan and Davison, Andrew J},
  journal={arXiv preprint arXiv:1612.05079},
  year={2016}
}

@inproceedings{geiger2012we,
  title={Are we ready for autonomous driving? the {KITTI} vision benchmark suite},
  author={Geiger, Andreas and Lenz, Philip and Urtasun, Raquel},
  booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3354--3361},
  year={2012},
}

@inproceedings{chang2019argoverse,
  title={Argoverse: 3{D} tracking and forecasting with rich maps},
  author={Chang, Ming-Fang and Lambert, John and Sangkloy, Patsorn and Singh, Jagjeet and Bak, Slawomir and Hartnett, Andrew and Wang, De and Carr, Peter and Lucey, Simon and Ramanan, Deva and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8748--8757},
  year={2019}
}

@inproceedings{de2013unsupervised,
  title={Unsupervised feature learning for classification of outdoor 3{D} scans},
  author={De Deuge, Mark and Quadros, Alastair and Hung, Calvin and Douillard, Bertrand},
  booktitle={Australasian Conference on Robitics and Automation},
  volume={2},
  pages={1},
  year={2013}
}


@inproceedings{caesar2020nuscenes,
  title={nu{S}cenes: A multimodal dataset for autonomous driving},
  author={Caesar, Holger and Bankiti, Varun and Lang, Alex H and Vora, Sourabh and Liong, Venice Erin and Xu, Qiang and Krishnan, Anush and Pan, Yu and Baldan, Giancarlo and Beijbom, Oscar},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={11621--11631},
  year={2020}
}

@article{tong2020cspc,
  title={{CSPC}-Dataset: New {LiDAR} Point Cloud Dataset and Benchmark for Large-Scale Scene Semantic Segmentation},
  author={Tong, Guofeng and Li, Yong and Chen, Dong and Sun, Qi and Cao, Wei and Xiang, Guiqiu},
  journal={IEEE Access},
  year={2020}
}

@inproceedings{Waymo,
  title={Scalability in perception for autonomous driving: Waymo open dataset},
  author={Sun, Pei and Kretzschmar, Henrik and Dotiwalla, Xerxes and Chouard, Aurelien and Patnaik, Vijaysai and Tsui, Paul and Guo, James and Zhou, Yin and Chai, Yuning and Caine, Benjamin and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2446--2454},
  year={2020}
}

@inproceedings{gaidon2016virtual,
  title={Virtual worlds as proxy for multi-object tracking analysis},
  author={Gaidon, Adrien and Wang, Qiao and Cabon, Yohann and Vig, Eleonora},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4340--4349},
  year={2016}
}

@inproceedings{ros2016synthia,
  title={The {SYNTHIA} dataset: A large collection of synthetic images for semantic segmentation of urban scenes},
  author={Ros, German and Sellart, Laura and Materzynska, Joanna and Vazquez, David and Lopez, Antonio M},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3234--3243},
  year={2016}
}

@article{geyer2020a2d2,
  title={A{2D}2: Audi autonomous driving dataset},
  author={Geyer, Jakob and Kassahun, Yohannes and Mahmudi, Mentar and Ricou, Xavier and Durgesh, Rupesh and Chung, Andrew S and Hauswald, Lorenz and Pham, Viet Hoang and M{\"u}hlegg, Maximilian and Dorn, Sebastian and others},
  journal={arXiv preprint arXiv:2004.06320},
  year={2020}
}

@inproceedings{le2018pointgrid,
  title={Point{G}rid: A deep network for 3{D} shape understanding},
  author={Le, Truc and Duan, Ye},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9204--9214},
  year={2018}
}

@article{Point-Voxel_CNN,
  title={Point-Voxel CNN for efficient 3{D} deep learning},
  author={Liu, Zhijian and Tang, Haotian and Lin, Yujun and Han, Song},
  journal={Advances in Neural Information Processing Systems},
  year={2019}
}

@article{vvnet,
  title={{VV-Net}: Voxel vae net with group convolutions for point cloud segmentation},
  author={Meng, Hsien-Yu and Gao, Lin and Lai, Yu-Kun and Manocha, Dinesh},
  journal={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{zhang2020polarnet,
  title={{PolarNet}: An Improved Grid Representation for Online {LiDAR} Point Clouds Semantic Segmentation},
  author={Zhang, Yang and Zhou, Zixiang and David, Philip and Yue, Xiangyu and Xi, Zerong and Gong, Boqing and Foroosh, Hassan},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9601--9610},
  year={2020}
}

@inproceedings{milioto2019rangenet++,
  title={Rangenet++: Fast and accurate {LiDAR} semantic segmentation},
  author={Milioto, Andres and Vizzo, Ignacio and Behley, Jens and Stachniss, Cyrill},
  booktitle={2019 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4213--4220},
  year={2019},
}

@inproceedings{lyu2020learning,
  title={Learning to Segment 3{D} Point Clouds in {2D} Image Space},
  author={Lyu, Yecheng and Huang, Xinming and Zhang, Ziming},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2020}
}

@article{cortinhal2020salsanext,
  title={Salsa{N}ext: Fast Semantic Segmentation of {LiDAR} Point Clouds for Autonomous Driving},
  author={Cortinhal, Tiago and Tzelepis, George and Aksoy, Eren Erdal},
  journal={arXiv preprint arXiv:2003.03653},
  year={2020}
}


@inproceedings{yan2020pointasnl,
  title={{PointASNL}: Robust Point Clouds Processing using Nonlocal Neural Networks with Adaptive Sampling},
  author={Yan, Xu and Zheng, Chaoda and Li, Zhen and Wang, Sheng and Cui, Shuguang},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={5589--5598},
  year={2020}
}

@inproceedings{zhou2018voxelnet,
  title={{VoxelNet}: End-to-end learning for point cloud based 3{D} object detection},
  author={Zhou, Yin and Tuzel, Oncel},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4490--4499},
  year={2018}
}

@article{votenet,
  title={Deep hough voting for 3{D} object detection in point clouds},
  author={Qi, Charles R and Litany, Or and He, Kaiming and Guibas, Leonidas J},
  journal={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9277--9286},
  year={2019}
}

@inproceedings{3D-MPA,
  title={3{D-MPA}: Multi-Proposal Aggregation for 3{D} Semantic Instance Segmentation},
  author={Engelmann, Francis and Bokeloh, Martin and Fathi, Alireza and Leibe, Bastian and Nie{\ss}ner, Matthias},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9031--9040},
  year={2020}
}

@inproceedings{handa2015scenenet,
  title={Scene{N}et: understanding real world indoor scenes with synthetic data},
  author={Handa, A and Patraucean, V and Badrinarayanan, V and Stent, S and Cipolla, R},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2016}
}

%%% PointNet %%%%%%%%%%%%%%%%%%%
@inproceedings{qi2017pointnet,
  title={{PointNet}: Deep learning on point sets for {3D} classification and segmentation},
  author={Qi, Charles R and Su, Hao and Mo, Kaichun and Guibas, Leonidas J},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={652--660},
  year={2017}
}

@article{qi2017pointnet++,
  title={Point{N}et++: Deep hierarchical feature learning on point sets in a metric space},
  author={Qi, Charles Ruizhongtai and Yi, Li and Su, Hao and Guibas, Leonidas J},
  journal={Advances in Neural Information Processing Systems},
  year={2017}
}


@inproceedings{Liu2019Point2SequenceLT,
  title={Point2sequence: Learning the shape representation of 3{D} point clouds with an attention-based sequence to sequence network},
  author={Liu, Xinhai and Han, Zhizhong and Liu, Yu-Shen and Zwicker, Matthias},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={8778--8785},
  year={2019}
}

@inproceedings{qi2018frustum,
  title={Frustum pointnets for {3D} object detection from {RGB-D} data},
  author={Qi, Charles R and Liu, Wei and Wu, Chenxia and Su, Hao and Guibas, Leonidas J},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={918--927},
  year={2018}
}

@inproceedings{shen2018mining,
  title={Mining point cloud local structures by kernel correlation and graph pooling},
  author={Shen, Yiru and Feng, Chen and Yang, Yaoqing and Tian, Dong},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4548--4557},
  year={2018}
}

%%% Graph-based %%%%%%%%%%%%%%%

@inproceedings{tchapmi2017segcloud,
  title={Segcloud: Semantic segmentation of {3D} point clouds},
  author={Tchapmi, Lyne and Choy, Christopher and Armeni, Iro and Gwak, JunYoung and Savarese, Silvio},
  booktitle={2017 International Conference on 3D Vision (3DV)},
  pages={537--547},
  year={2017},
}

@article{dgcnn,
  title={Dynamic graph cnn for learning on point clouds},
  author={Wang, Yue and Sun, Yongbin and Liu, Ziwei and Sarma, Sanjay E and Bronstein, Michael M and Solomon, Justin M},
  journal={ACM Transactions On Graphics (TOG)},
  volume={38},
  number={5},
  pages={1--12},
  year={2019},
}

@inproceedings{landrieu2018large,
  title={Large-scale point cloud semantic segmentation with superpoint graphs},
  author={Landrieu, Loic and Simonovsky, Martin},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4558--4567},
  year={2018}
}

@inproceedings{landrieu2019point,
  title={Point Cloud Oversegmentation with Graph-Structured Deep Metric Learning},
  author={Landrieu, Loic and Boussaha, Mohamed},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={7440--7449},
  year={2019}
}

@inproceedings{wang2019graph,
  title={Graph Attention Convolution for Point Cloud Semantic Segmentation},
  author={Wang, Lei and Huang, Yuchun and Hou, Yaolin and Zhang, Shenman and Shan, Jie},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={10296--10305},
  year={2019}
}

@article{li2018pointcnn,
  title={{PointCNN}: Convolution on {X}-transformed points},
  author={Li, Yangyan and Bu, Rui and Sun, Mingchao and Wu, Wei and Di, Xinhan and Chen, Baoquan},
  journal={Advances in Neural Information Processing Systems},
  year={2018}
}

@inproceedings{wang2018deep,
  title={Deep parametric continuous convolutional neural networks},
  author={Wang, Shenlong and Suo, Simon and Ma, Wei-Chiu and Pokrovsky, Andrei and Urtasun, Raquel},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2589--2597},
  year={2018}
}

@article{Groh2018flexconv,
  author    = {Fabian Groh and
               Patrick Wieschollek and
               Hendrik P. A. Lensch
               },
  title     = {Flex-Convolution (Million-Scale Point-Cloud Learning Beyond Grid-Worlds)},
  journal = {ACCV},
  year      = {2018}
}



@inproceedings{zhang2018efficient,
  title={Efficient Convolutions for Real-Time Semantic Segmentation of 3{D} Point Clouds},
  author={Zhang, Chris and Luo, Wenjie and Urtasun, Raquel},
  booktitle={2018 International Conference on 3D Vision (3DV)},
  pages={399--408},
  year={2018},
}

%%% voxels %%%%%%%%%%%%%%%%
@inproceedings{riegler2017octnet,
  title={Oct{N}et: Learning deep {3D} representations at high resolutions},
  author={Riegler, Gernot and Osman Ulusoy, Ali and Geiger, Andreas},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3577--3586},
  year={2017}
}

@inproceedings{wu20153d,
  title={{3D} shapenets: A deep representation for volumetric shapes},
  author={Wu, Zhirong and Song, Shuran and Khosla, Aditya and Yu, Fisher and Zhang, Linguang and Tang, Xiaoou and Xiao, Jianxiong},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1912--1920},
  year={2015}
}


@inproceedings{boulch2017unstructured,
  title={Unstructured point cloud semantic labeling using deep segmentation networks},
  author={Boulch, A and Saux, B Le and Audebert, N},
  booktitle={Proceedings of the Workshop on 3D Object Retrieval},
  pages={17--24},
  year={2017}
}


@article{boulch2019generalizing,
  title={Generalizing discrete convolutions for unstructured point clouds},
  author={Boulch, Alexandre},
  journal={arXiv preprint arXiv:1904.02375},
  year={2019}
}

%%% Attention %%%%%%%%%%%%%%
@article{bahdanau2014neural,
  title={Neural machine translation by jointly learning to align and translate},
  author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1409.0473},
  year={2014}
}
@article{xu2015show,
  title={Show, attend and tell: Neural image caption generation with visual attention},
  author={Xu, Kelvin and Ba, Jimmy and Kiros, Ryan and Cho, Kyunghyun and Courville, Aaron and Salakhudinov, Ruslan and Zemel, Rich and Bengio, Yoshua},
  journal={ICML},
  year={2015}
}
@article{lu2016hierarchical,
  title={Hierarchical question-image co-attention for visual question answering},
  author={Lu, Jiasen and Yang, Jianwei and Batra, Dhruv and Parikh, Devi},
  journal={Advances in Neural Information Processing Systems},
  year={2016}
}


@inproceedings{wang2017coupled,
  title={Coupled multi-layer attentions for co-extraction of aspect and opinion terms},
  author={Wang, Wenya and Pan, Sinno Jialin and Dahlmeier, Daniel and Xiao, Xiaokui},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={31},
  number={1},
  year={2017}
}

@article{lee2017interactive,
  title={Interactive visualization and manipulation of attention-based neural machine translation},
  author={Lee, Jaesong and Shin, Joong-Hwi and Kim, Jun-Seok},
  journal={EMNLP},
  year={2017}
}

@inproceedings{Yang2019ModelingPC,
  title={Modeling Point Clouds with Self-Attention and Gumbel Subset Sampling},
  author={Yang, Jiancheng and Zhang, Qiang and Ni, Bingbing and Li, Linguo and Liu, Jinxian and Zhou, Mengdie and Tian, Qi},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@article{chen2019lsanet,
  title={{LSAN}et: Feature Learning on Point Sets by Local Spatial Attention},
  author={Chen, Lin-Zhuo and Li, Xuan-Yi and Fan, Deng-Ping and Cheng, Ming-Ming and Wang, Kai and Lu, Shao-Ping},
  journal={arXiv preprint arXiv:1905.05442},
  year={2019}
}
@article{chen2019gapnet,
  title={GAPNet: Graph Attention based Point Neural Network for Exploiting Local Feature of Point Cloud},
  author={Chen, Can and Fragonara, Luca Zanotti and Tsourdos, Antonios},
  journal={arXiv preprint arXiv:1905.08705},
  year={2019}
}
@article{xie2019point,
  title={Point Clouds Learning with Attention-based Graph Convolution Networks},
  author={Xie, Zhuyang and Chen, Junzhou and Peng, Bo},
  journal={arXiv preprint arXiv:1905.13445},
  year={2019}
}
@article{zhiheng2019pyramnet,
  title={PyramNet: Point Cloud Pyramid Attention Network and Graph Embedding Module for Classification and Segmentation},
  author={Zhiheng, Kang and Ning, Li},
  journal={arXiv preprint arXiv:1906.03299},
  year={2019}
}
@inproceedings{xie2018attentional,
  title={Attentional shapecontextnet for point cloud recognition},
  author={Xie, Saining and Liu, Sainan and Chen, Zeyu and Tu, Zhuowen},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}



%%% Other %%%%%%%%%%%%%%%
@article{Choy20194DSC,
  title={4{D} Spatio-Temporal ConvNets: Minkowski Convolutional Neural Networks},
  author={Christopher Bongsoo Choy and JunYoung Gwak and Silvio Savarese},
  journal={CoRR},
  year={2019},
  volume={abs/1904.08755}
}

@article{wu2019fastfcn,
  title     = {FastFCN: Rethinking Dilated Convolution in the Backbone for Semantic Segmentation},
  author    = {Wu, Huikai and Zhang, Junge and Huang, Kaiqi and Liang, Kongming and Yu Yizhou},
  journal = {arXiv preprint arXiv:1903.11816},
  year = {2019}
}

@article{yang2018attentional,
  title={Attentional Aggregation of Deep Feature Sets for Multi-view {3D} Reconstruction},
  author={Yang, Bo and Wang, Sen and Markham, Andrew and Trigoni, Niki},
  journal={arXiv preprint arXiv:1808.00758},
  year={2018}
}

@article{thomas2018semantic,
  title={Semantic Classification of {3D} Point Clouds with Multiscale Spherical Neighborhoods},
  author={Thomas, Hugues and Goulette, Fran{\c{c}}ois and Deschaud, Jean-Emmanuel and Marcotegui, Beatriz},
  journal={3DV},
  year={2018},
}

@inproceedings{simonovsky2017dynamic,
  title={Dynamic edge-conditioned filters in convolutional neural networks on graphs},
  author={Simonovsky, Martin and Komodakis, Nikos},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2017}
}

@article{Xie_2018_CVPR,
author = {Xie, Saining and Liu, Sainan and Chen, Zeyu and Tu, Zhuowen},
title = {Attentional ShapeContextNet for Point Cloud Recognition},
journal = {CVPR},
month = {June},
year = {2018}
}

@inproceedings{huang2018recurrent,
  title={Recurrent slice networks for 3{D} segmentation of point clouds},
  author={Huang, Qiangui and Wang, Weiyue and Neumann, Ulrich},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@inproceedings{xu2018spidercnn,
  title={Spidercnn: Deep learning on point sets with parameterized convolutional filters},
  author={Xu, Yifan and Fan, Tianqi and Xu, Mingye and Zeng, Long and Qiao, Yu},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  year={2018}
}

@inproceedings{engelmann2018know,
  title={Know what your neighbors do: 3{D} semantic segmentation of point clouds},
  author={Engelmann, Francis and Kontogianni, Theodora and Schult, Jonas and Leibe, Bastian},
  booktitle={Proceedings of the European Conference on Computer Vision Workshop (ECCV)},
  year={2018}
}

@misc{Lyft,
  title = {Lyft Level 5 Dataset},
  howpublished = {\url{https://self-driving.lyft.com/level5/data/}},
}


%%% datasets %%%%%%%%%%%%%%%%%%%%%%%
@inproceedings{2D-3D-S,
  title={Joint 2{D}-3{D}-semantic data for indoor scene understanding},
  author={Armeni, Iro and Sax, Sasha and Zamir, Amir R and Savarese, Silvio},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2017}
}


@article{Semantic3D,
  title={Semantic3{D}.{N}et: A new large-scale point cloud classification benchmark},
  author={Hackel, Timo and Savinov, Nikolay and Ladicky, Lubor and Wegner, Jan D and Schindler, Konrad and Pollefeys, Marc},
  journal={ISPRS Annals of Photogrammetry, Remote Sensing \& Spatial Information Sciences},
  year={2017}
}

@article{grilli2017review,
  title={A review of point clouds segmentation and classification algorithms},
  author={Grilli, E and Menna, F and Remondino, F},
  journal={The International Archives of Photogrammetry, Remote Sensing and Spatial Information Sciences},
  volume={42},
  year={2017},
  publisher={Copernicus GmbH}
}

@article{nguyen2013survey,
  title={{3D} point cloud segmentation: A survey},
  author={Nguyen, Anh and Le, Bac},
  journal={2013 6th IEEE conference on robotics, automation and mechatronics},
  year={2013},
}

@inproceedings{engelmann2017exploring,
  title={Exploring spatial context for 3{D} semantic segmentation of point clouds},
  author={Engelmann, Francis and Kontogianni, Theodora and Hermans, Alexander and Leibe, Bastian},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision Workshops},
  pages={716--724},
  year={2017}
}

@inproceedings{3PRNN,
  title={{3D} recurrent neural networks with context fusion for point cloud semantic segmentation},
  author={Ye, Xiaoqing and Li, Jiamao and Huang, Hexiao and Du, Liang and Zhang, Xiaolin},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  year={2018}
}

@inproceedings{RSNet,
  title={Recurrent slice networks for {3D} segmentation of point clouds},
  author={Huang, Qiangui and Wang, Weiyue and Neumann, Ulrich},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@article{pedro,
  title={Monte Carlo convolution for learning on non-uniformly sampled point clouds},
  author={Hermosilla, Pedro and Ritschel, Tobias and V{\'a}zquez, Pere-Pau and Vinacua, {\`A}lvar and Ropinski, Timo},
  journal={SIGGRAPH Asia 2018 Technical Papers},
  year={2018},
}

@article{thomas2019kpconv,
  title={{KPConv}: Flexible and Deformable Convolution for Point Clouds},
  author={Thomas, Hugues and Qi, Charles R and Deschaud, Jean-Emmanuel and Marcotegui, Beatriz and Goulette, Fran{\c{c}}ois and Guibas, Leonidas J},
  journal={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={6411--6420},
  year={2019}
}

@inproceedings{liu2019relation,
  title={Relation-Shape Convolutional Neural Network for Point Cloud Analysis},
  author={Liu, Yongcheng and Fan, Bin and Xiang, Shiming and Pan, Chunhong},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{wu2018pointconv,
  title={{PointConv}: Deep Convolutional Networks on 3{D} Point Clouds},
  author={Wu, Wenxuan and Qi, Zhongang and Fuxin, Li},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9621--9630},
  year={2018}
}

@inproceedings{so-net,
  title={{SO-Net}: Self-organizing network for point cloud analysis},
  author={Li, Jiaxin and Chen, Ben M and Hee Lee, Gim},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@inproceedings{Geo-CNN,
  title={{Modeling local geometric structure of 3{D} point clouds using Geo-CNN}},
  author={Lan, Shiyi and Yu, Ruichi and Yu, Gang and Davis, Larry S},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{KCNet,
  title={Mining point cloud local structures by kernel correlation and graph pooling},
  author={Shen, Yiru and Feng, Chen and Yang, Yaoqing and Tian, Dong},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@inproceedings{su2018splatnet,
  title={{SPLATNet:} Sparse lattice networks for point cloud processing},
  author={Su, Hang and Jampani, Varun and Sun, Deqing and Maji, Subhransu and Kalogerakis, Evangelos and Yang, Ming-Hsuan and Kautz, Jan},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2530--2539},
  year={2018}
}

@inproceedings{rethage2018fully,
  title={Fully-convolutional point networks for large-scale point clouds},
  author={Rethage, Dario and Wald, Johanna and Sturm, Jurgen and Navab, Nassir and Tombari, Federico},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  year={2018}
}


@article{conv_pts,
  title={Generalizing discrete convolutions for unstructured point clouds},
  author={Boulch, Alexandre},
  journal={arXiv preprint arXiv:1904.02375},
  year={2019}
}


@article{TMLC-MS,
  title={Fast semantic segmentation of 3{D} point clouds with strongly varying density},
  author={Hackel, Timo and Wegner, Jan D and Schindler, Konrad},
  journal={ISPRS annals of the photogrammetry, remote sensing and spatial information sciences},
  volume={3},
  pages={177--184},
  year={2016},
}

@inproceedings{GACNet,
  title={Graph Attention Convolution for Point Cloud Semantic Segmentation},
  author={Wang, Lei and Huang, Yuchun and Hou, Yaolin and Zhang, Shenman and Shan, Jie},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}


@inproceedings{AttentionalPointNet,
  title={Attentional PointNet for 3D-Object Detection in Point Clouds},
  author={Paigwar, Anshul and Erkent, Ozgur and Wolf, Christian and Laugier, Christian},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={0--0},
  year={2019}
}

@inproceedings{PCAN,
  title={{PCAN}: {3D} Attention Map Learning Using Contextual Information for Point Cloud Based Retrieval},
  author={Zhang, Wenxiao and Xiao, Chunxia},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2016}
}

@inproceedings{snapnet,
  title={Unstructured point cloud semantic labeling using deep segmentation networks},
  author={Boulch, A and Saux, B Le and Audebert, N},
  booktitle={Proceedings of the Workshop on 3D Object Retrieval},
  pages={17--24},
  year={2017}
}


@article{msdeepvoxnet,
  title={Classification of point cloud scenes with multiscale voxel deep network},
  author={Roynard, Xavier and Deschaud, Jean-Emmanuel and Goulette, Fran{\c{c}}ois},
  journal={arXiv preprint arXiv:1804.03583},
  year={2018}
}


@inproceedings{RF_MSSF,
  title={Semantic classification of 3{D} point clouds with multiscale spherical neighborhoods},
  author={Thomas, Hugues and Goulette, Fran{\c{c}}ois and Deschaud, Jean-Emmanuel and Marcotegui, Beatriz and LeGall, Yann},
  booktitle={2018 International conference on 3D Vision (3DV)},
  pages={390--398},
  year={2018},
}


@inproceedings{wu2018squeezeseg,
  title={Squeeze{S}eg: Convolutional neural nets with recurrent {CRF} for real-time road-object segmentation from 3{D} {LiDAR} point cloud},
  author={Wu, Bichen and Wan, Alvin and Yue, Xiangyu and Keutzer, Kurt},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={1887--1893},
  year={2018},
}

@inproceedings{wu2019squeezesegv2,
  title={Squeezesegv2: Improved model structure and unsupervised domain adaptation for road-object segmentation from a {LiDAR} point cloud},
  author={Wu, Bichen and Zhou, Xuanyu and Zhao, Sicheng and Yue, Xiangyu and Keutzer, Kurt},
  booktitle={2019 International Conference on Robotics and Automation (ICRA)},
  pages={4376--4382},
  year={2019},
}

@inproceedings{tangentconv,
  title={Tangent convolutions for dense prediction in 3{D}},
  author={Tatarchenko, Maxim and Park, Jaesik and Koltun, Vladlen and Zhou, Qian-Yi},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3887--3896},
  year={2018}
}

@inproceedings{behley2019semantickitti,
  title={{SemanticKITTI}: A Dataset for Semantic Scene Understanding of {LiDAR} Sequences},
  author={Behley, Jens and Garbade, Martin and Milioto, Andres and Quenzel, Jan and Behnke, Sven and Stachniss, Cyrill and Gall, Jurgen},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9297--9307},
  year={2019}
}

@article{zhang2019shellnet,
  title={Shell{N}et: Efficient Point Cloud Convolutional Neural Networks using Concentric Shells Statistics},
  author={Zhang, Zhiyuan and Hua, Binh-Son and Yeung, Sai-Kit},
  journal={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1607--1616},
  year={2019}
}

@article{yolov3,
  title={Yolov3: An incremental improvement},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}

@inproceedings{SRN,
  title={Structural Relational Reasoning of Point Clouds},
  author={Duan, Yueqi and Zheng, Yu and Lu, Jiwen and Zhou, Jie and Tian, Qi},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@article{DPC,
  title={Dilated Point Convolutions: On the Receptive Field of Point Convolutions},
  author={Engelmann, Francis and Kontogianni, Theodora and Leibe, Bastian},
  journal={BMVC},
  year={2019}
}

@inproceedings{learning2sample,
  title={Learning to Sample},
  author={Dovrat, Oren and Lang, Itai and Avidan, Shai},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@article{concrete,
  title={Concrete Autoencoders for Differentiable Feature Selection and Reconstruction},
  author={Abid, Abubakar and Balin, Muhammad Fatih and Zou, James},
  journal={ICML},
  year={2019}
}

@inproceedings{scannet,
  title={Scan{N}et: Richly-annotated 3{D} reconstructions of indoor scenes},
  author={Dai, Angela and Chang, Angel X and Savva, Manolis and Halber, Maciej and Funkhouser, Thomas and Nie{\ss}ner, Matthias},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={5828--5839},
  year={2017}
}

@article{zhao2019ps,
  title={PS\^{} 2-Net: A Locally and Globally Aware Network for Point-Based Semantic Segmentation},
  author={Zhao, Na and Chua, Tat-Seng and Lee, Gim Hee},
  journal={arXiv preprint arXiv:1908.05425},
  year={2019}
}

@article{3dbonet,
  title={Learning Object Bounding Boxes for 3{D} Instance Segmentation on Point Clouds},
  author={Yang, Bo and Wang, Jianan and Clark, Ronald and Hu, Qingyong and Wang, Sen and Markham, Andrew and Trigoni, Niki},
  journal={Advances in Neural Information Processing Systems},
  year={2019}
}

@inproceedings{sparse,
  title={3{D} semantic segmentation with submanifold sparse convolutional networks},
  author={Graham, Benjamin and Engelcke, Martin and van der Maaten, Laurens},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@article{concrete_distribution,
  title={The concrete distribution: A continuous relaxation of discrete random variables},
  author={Maddison, Chris J and Mnih, Andriy and Teh, Yee Whye},
  journal={arXiv preprint arXiv:1611.00712},
  year={2016}
}

@article{show_attend,
  title={Show, attend and tell: Neural image caption generation with visual attention},
  author={Xu, Kelvin and Ba, Jimmy and Kiros, Ryan and Cho, Kyunghyun and Courville, Aaron and Salakhudinov, Ruslan and Zemel, Rich and Bengio, Yoshua},
  journal={ICML},
  year={2015}
}

@inproceedings{pointgrid,
  title={{PointGrid}: A deep network for 3{D} shape understanding},
  author={Le, Truc and Duan, Ye},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@inproceedings{HPEIN,
author = {Jiang, Li and Zhao, Hengshuang and Liu, Shu and Shen, Xiaoyong and Fu, Chi-Wing and Jia, Jiaya},
title = {Hierarchical Point-Edge Interaction Network for Point Cloud Semantic Segmentation},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision},
year = {2019}
}

@inproceedings{pointweb,
  title={PointWeb: Enhancing Local Neighborhood Features for Point Cloud Processing},
  author={Zhao, Hengshuang and Jiang, Li and Fu, Chi-Wing and Jia, Jiaya},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{local_spectral,
  title={Local spectral graph convolution for point set feature learning},
  author={Wang, Chu and Samari, Babak and Siddiqi, Kaleem},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  year={2018}
}

@inproceedings{clusternet,
  title={Cluster{N}et: Deep Hierarchical Cluster Network with Rigorously Rotation-Invariant Representation for Point Cloud Analysis},
  author={Chen, Chao and Li, Guanbin and Xu, Ruijia and Chen, Tianshui and Wang, Meng and Lin, Liang},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{Agglomeration,
author = {Liu, Jinxian and Ni, Bingbing and Li, Caiyuan and Yang, Jiancheng and Tian, Qi},
title = {Dynamic Points Agglomeration for Hierarchical Point Sets Learning},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision},
year = {2019}
}

@inproceedings{hua2018pointwise,
  title={Pointwise convolutional neural networks},
  author={Hua, Binh-Son and Tran, Minh-Khoi and Yeung, Sai-Kit},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@inproceedings{octree_guided,
  title={Octree guided CNN with Spherical Kernels for 3{D} Point Clouds},
  author={Lei, Huan and Akhtar, Naveed and Mian, Ajmal},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{ACNN,
  title={{A-CNN}: Annularly Convolutional Neural Networks on Point Clouds},
  author={Komarichev, Artem and Zhong, Zichun and Hua, Jing},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@article{mao2019interpolated,
  title={Interpolated Convolutional Networks for 3{D} Point Cloud Understanding},
  author={Mao, Jiageng and Wang, Xiaogang and Li, Hongsheng},
  journal={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}


@inproceedings{PCT,
  title={PCT: Large-scale 3{D} point cloud representations via graph inception networks with applications to autonomous driving},
  author={Chen, Siheng and Niu, Sufeng and Lan, Tian and Liu, Baoan},
  booktitle={2019 IEEE International Conference on Image Processing (ICIP)},
  pages={4395--4399},
  year={2019},
}

 
@article{point_signatures,
  title={Point signatures: A new representation for 3{D} object recognition},
  author={Chua, Chin Seng and Jarvis, Ray},
  journal={International Journal of Computer Vision},
  volume={25},
  number={1},
  pages={63--85},
  year={1997},
}



@inproceedings{fast_hist,
  title={Fast point feature histograms (FPFH) for 3{D} registration},
  author={Rusu, Radu Bogdan and Blodow, Nico and Beetz, Michael},
  booktitle={2009 IEEE international conference on robotics and automation},
  pages={3212--3217},
  year={2009},
}

@article{li2016vehicle_rss,
  title={Vehicle detection from 3{D} {LiDAR} using fully convolutional network},
  author={Li, Bo and Zhang, Tianlei and Xia, Tian},
  journal={RSS},
  year={2016}
}

@inproceedings{chen2017multi,
  title={Multi-view 3{D} object detection network for autonomous driving},
  author={Chen, Xiaozhi and Ma, Huimin and Wan, Ji and Li, Bo and Xia, Tian},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2017}
}

@inproceedings{PIXOR,
  title={Pixor: Real-time 3{D} object detection from point clouds},
  author={Yang, Bin and Luo, Wenjie and Urtasun, Raquel},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2018}
}

@inproceedings{pointpillars,
  title={{PointPillars}: Fast encoders for object detection from point clouds},
  author={Lang, Alex H and Vora, Sourabh and Caesar, Holger and Zhou, Lubing and Yang, Jiong and Beijbom, Oscar},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@inproceedings{4dMinkpwski,
  title={4{D} Spatio-Temporal ConvNets: Minkowski Convolutional Neural Networks},
  author={Choy, Christopher and Gwak, JunYoung and Savarese, Silvio},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3075--3084},
  year={2019}
}


@inproceedings{Fast_point_rcnn,
author = {Chen, Yilun and Liu, Shu and Shen, Xiaoyong and Jia, Jiaya},
title = {Fast Point {R-CNN}},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision},
year = {2019}
}


@article{Yang_ijcv2019,
  title={Robust attentional aggregation of deep feature sets for multi-view 3{D} reconstruction},
  author={Yang, Bo and Wang, Sen and Markham, Andrew and Trigoni, Niki},
  journal={International Journal of Computer Vision},
  volume={128},
  number={1},
  pages={53--73},
  year={2020},
}

@article{liu2019meteornet,
  title={{MeteorNet}: Deep Learning on Dynamic 3{D} Point Cloud Sequences},
  author={Liu, Xingyu and Yan, Mengyuan and Bohg, Jeannette},
  journal={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2019}
}

@article{sutton2000policy,
  title={Policy gradient methods for reinforcement learning with function approximation},
  author={Sutton, Richard S and McAllester, David A and Singh, Satinder P and Mansour, Yishay},
  journal={Advances in Neural Information Processing Systems},
  year={2000}
}

@article{mnih2014neural,
  title={Neural variational inference and learning in belief networks},
  author={Mnih, Andriy and Gregor, Karol},
  journal={arXiv preprint arXiv:1402.0030},
  year={2014}
}


@article{landrieu2017structured,
  title={A structured regularization framework for spatially smoothing semantic labelings of 3{D} point clouds},
  author={Landrieu, Loic and Raguet, Hugo and Vallet, Bruno and Mallet, Cl{\'e}ment and Weinmann, Martin},
  journal={ISPRS Journal of Photogrammetry and Remote Sensing},
  volume={132},
  pages={102--118},
  year={2017},
}


@article{hackel2016fast,
  title={Fast semantic segmentation of 3{D} point clouds with strongly varying density},
  author={Hackel, Timo and Wegner, Jan D and Schindler, Konrad},
  journal={ISPRS annals of the photogrammetry, remote sensing and spatial information sciences},
  volume={3},
  pages={177--184},
  year={2016},
}


@inproceedings{rangenet++,
  title={Rangenet++: Fast and accurate {LiDAR} semantic segmentation},
  author={Milioto, Andres and Vizzo, Ignacio and Behley, Jens and Stachniss, Cyrill},
  booktitle={2019 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4213--4220},
  year={2019},
}

@inproceedings{Li_2019_ICCV,
author = {Li, Guohao and Muller, Matthias and Thabet, Ali and Ghanem, Bernard},
title = {DeepGCNs: Can GCNs Go As Deep As CNNs?},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision},
year = {2019}
}

@article{guo2019deep,
  title={Deep Learning for 3{D} Point Clouds: A Survey},
  author={Guo, Yulan and Wang, Hanyun and Hu, Qingyong and Liu, Hao and Liu, Li and Bennamoun, Mohammed},
  journal={IEEE TPAMI},
  year={2020}
}

@article{Point_voxel_cnn,
  title={Point-Voxel CNN for efficient 3{D} deep learning},
  author={Liu, Zhijian and Tang, Haotian and Lin, Yujun and Han, Song},
  journal={Advances in Neural Information Processing Systems},
  year={2019}
}


@inproceedings{Toronto3D,
  title={Toronto-3{D}: A Large-scale Mobile {LiDAR} Dataset for Semantic Segmentation of Urban Roadways},
  author={Tan, Weikai and Qin, Nannan and Ma, Lingfei and Li, Ying and Du, Jing and Cai, Guorong and Yang, Ke and Li, Jonathan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={202--203},
  year={2020}
}

@article{ma2019multi,
  title={Multi-Scale Point-Wise Convolutional Neural Networks for 3{D} Object Segmentation From {LiDAR} Point Clouds in Large-Scale Environments},
  author={Ma, Lingfei and Li, Ying and Li, Jonathan and Tan, Weikai and Yu, Yongtao and Chapman, Michael A},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  year={2019},
}

@article{li2019tgnet,
  title={TGNet: Geometric Graph CNN on 3-D Point Cloud Segmentation},
  author={Li, Ying and Ma, Lingfei and Zhong, Zilong and Cao, Dongpu and Li, Jonathan},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  year={2019},
}


@inproceedings{RGNet,
  title={Fast Point Cloud Registration using Semantic Segmentation},
  author={Truong, Giang and Gilani, Syed Zulqarnain and Islam, Syed Mohammed Shamsul and Suter, David},
  booktitle={2019 Digital Image Computing: Techniques and Applications (DICTA)},
  pages={1--8},
  year={2019},
}

@article{rosu2019latticenet,
  title={Lattice{N}et: Fast point cloud segmentation using permutohedral lattices},
  author={Rosu, Radu Alexandru and Sch{\"u}tt, Peer and Quenzel, Jan and Behnke, Sven},
  journal={arXiv preprint arXiv:1912.05905},
  year={2019}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{MS3DVS,
  title={Classification of Point Cloud for Road Scene Understanding with Multiscale Voxel Deep Network},
  author={Roynard, Xavier and Deschaud, Jean-Emmanuel and Goulette, Fran{\c{c}}ois},
  journal={10th workshop on Planning, Perceptionand Navigation for Intelligent Vehicules PPNIV'2018},
  year={2018}
}


@inproceedings{liang2019hierarchical,
  title={Hierarchical depthwise graph convolutional neural network for 3{D} semantic segmentation of point clouds},
  author={Liang, Zhidong and Yang, Ming and Deng, Liuyuan and Wang, Chunxiang and Wang, Bing},
  booktitle={2019 International Conference on Robotics and Automation (ICRA)},
  pages={8152--8158},
  year={2019},
}

@article{boulch2020lightconvpoint,
  title={LightConvPoint: convolution for points},
  author={Boulch, Alexandre and Puy, Gilles and Marlet, Renaud},
  journal={arXiv preprint arXiv:2004.04462},
  year={2020}
}

@article{NPM3D,
  title={{Paris-Lille-3D}: A large and high-quality ground-truth urban point cloud dataset for automatic segmentation and classification},
  author={Roynard, Xavier and Deschaud, Jean-Emmanuel and Goulette, Fran{\c{c}}ois},
  journal={The International Journal of Robotics Research},
  volume={37},
  number={6},
  pages={545--557},
  year={2018},
}

@article{salsanext,
  title={SalsaNext: Fast Semantic Segmentation of {LiDAR} Point Clouds for Autonomous Driving},
  author={Cortinhal, Tiago and Tzelepis, George and Aksoy, Eren Erdal},
  journal={arXiv preprint arXiv:2003.03653},
  year={2020}
}

@inproceedings{xu2020squeezesegv3,
  title={Squeeze{S}eg{V}3: Spatially-Adaptive Convolution for Efficient Point-Cloud Segmentation},
  author={Xu, Chenfeng and Wu, Bichen and Wang, Zining and Zhan, Wei and Vajda, Peter and Keutzer, Kurt and Tomizuka, Masayoshi},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={1--19},
  year={2020}
}

@article{montoya2014mind,
  title={{Mind the gap: modeling local and global context in (road) networks}},
  author={Montoya-Zegarra, Javier A and Wegner, Jan D and Ladick{\`y}, L'ubor and Schindler, Konrad},
  journal={German Conference on Pattern Recognition},
  year={2014},
}


@inproceedings{contreras2019edge,
  title={Edge-convolution point net for semantic segmentation of large-scale point clouds},
  author={Contreras, Jhonatan and Denzler, Joachim},
  booktitle={IGARSS 2019-2019 IEEE International Geoscience and Remote Sensing Symposium},
  pages={5236--5239},
  year={2019},
}

@article{ma2020global,
  title={Global Context Reasoning for Semantic Segmentation of 3{D} Point Clouds},
  author={Ma, Yanni and Guo, Yulan and Liu, Hao and Lei, Yinjie and Wen, Gongjian},
  journal={WACV},
  year={2020}
}

@inproceedings{hu2019randla,
  title={{RandLA-Net}: Efficient Semantic Segmentation of Large-Scale Point Clouds},
  author={Hu, Qingyong and Yang, Bo and Xie, Linhai and Rosa, Stefano and Guo, Yulan and Wang, Zhihua and Trigoni, Niki and Markham, Andrew},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2020}
}


@inproceedings{varney2020dales,
  title={{DALES}: A Large-scale Aerial {LiDAR} Data Set for Semantic Segmentation},
  author={Varney, Nina and Asari, Vijayan K and Graehling, Quinn},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={186--187},
  year={2020}
}

@article{pan2020semanticposs,
  title={SemanticPOSS: A Point Cloud Dataset with Large Quantity of Dynamic Instances},
  author={Pan, Yancheng and Gao, Biao and Mei, Jilin and Geng, Sibo and Li, Chengkun and Zhao, Huijing},
  journal={arXiv preprint arXiv:2002.09147},
  year={2020}
}


@article{rottensteiner2012isprs,
  title={The {ISPRS} benchmark on urban object classification and 3{D} building reconstruction},
  author={Rottensteiner, Franz and Sohn, Gunho and Jung, Jaewook and Gerke, Markus and Baillard, Caroline and Benitez, Sebastien and Breitkopf, Uwe},
  journal={ISPRS Annals of the Photogrammetry, Remote Sensing and Spatial Information Sciences I-3 (2012), Nr. 1},
  volume={1},
  number={1},
  pages={293--298},
  year={2012},
}

@inproceedings{oakland,
  title={Contextual classification with functional max-margin markov networks},
  author={Munoz, Daniel and Bagnell, J Andrew and Vandapel, Nicolas and Hebert, Martial},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2009},
}


@article{IQmulus,
  title={{TerraMobilita/iQmulus} urban point cloud analysis benchmark},
  author={Vallet, Bruno and Br{\'e}dif, Mathieu and Serna, Andr{\'e}s and Marcotegui, Beatriz and Paparoditis, Nicolas},
  journal={Computers \& Graphics},
  year={2015},
}


@inproceedings{paris-rue-madame,
  title={Paris-rue-Madame database: a 3{D} mobile laser scanner dataset for benchmarking urban detection, segmentation and classification methods},
  author={Serna, Andr{\'e}s and Marcotegui, Beatriz and Goulette, Fran{\c{c}}ois and Deschaud, Jean-Emmanuel},
  booktitle={4th International Conference on Pattern Recognition, Applications and Methods ICPRAM 2014},
  year={2014}
}

@article{Sydney_urban,
  title={Representing 3{D} shape in sparse range images for urban object classification},
  author={Quadros, Alistair James},
  year={2013},
  publisher={University of Sydney.}
}

@article{focal_loss,
  title={Focal loss for dense object detection},
  author={Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
  journal={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  year={2017}
}

@inproceedings{berman2018lovasz,
  title={The lov{\'a}sz-softmax loss: a tractable surrogate for the optimization of the intersection-over-union measure in neural networks},
  author={Berman, Maxim and Rannen Triki, Amal and Blaschko, Matthew B},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4413--4421},
  year={2018}
}



@incollection{generalised_dice,
  title={Generalised dice overlap as a deep learning loss function for highly unbalanced segmentations},
  author={Sudre, Carole H and Li, Wenqi and Vercauteren, Tom and Ourselin, Sebastien and Cardoso, M Jorge},
  journal={Deep learning in medical image analysis and multimodal learning for clinical decision support},
  year={2017},
}


@article{3d_modeling,
  title={3{D} urban scene modeling integrating recognition and reconstruction},
  author={Cornelis, Nico and Leibe, Bastian and Cornelis, Kurt and Van Gool, Luc},
  journal={International Journal of Computer Vision},
  volume={78},
  number={2-3},
  pages={121--141},
  year={2008},
}


@inproceedings{salsanet,
  title={Salsanet: Fast road and vehicle segmentation in {LiDAR} point clouds for autonomous driving},
  author={Aksoy, Eren Erdal and Baci, Saimir and Cavdar, Selcuk},
  booktitle={IEEE Intelligent Vehicles Symposium (IV)},
  pages={926--932},
  year={2019},
}


@inproceedings{zolanvari2019dublincity,
  title={Dublin{C}ity: Annotated {LiDAR} Point Cloud and its Applications},
  author={Zolanvari, SM and Ruano, Susana and Rana, Aakanksha and Cummins, Alan and da Silva, Rogerio Eduardo and Rahbar, Morteza and Smolic, Aljosa},
  booktitle={British Machine Vision Conference},
  year={2019}
}

@article{li2020campus3d,
  title={Campus3{D}: A photogrammetry point cloud benchmark for hierarchical understanding of outdoor scene},
  author={Li, Xinke and Li, Chongshou and Tong, Zekun and Lim, Andrew and Yuan, Junsong and Wu, Yuwei and Tang, Jing and Huang, Raymond},
  journal={ACM MM},
  year={2020}
}

@article{ye2020lasdu,
  title={{LASDU}: A Large-Scale Aerial {LiDAR} Dataset for Semantic Labeling in Dense Urban Areas},
  author={Ye, Zhen and Xu, Yusheng and Huang, Rong and Tong, Xiaohua and Li, Xin and Liu, Xiangfeng and Luan, Kuifeng and Hoegner, Ludwig and Stilla, Uwe},
  journal={ISPRS International Journal of Geo-Information},
  volume={9},
  number={7},
  pages={450},
  year={2020},
}

@article{zhang2018patch,
  title={A patch-based method for the evaluation of dense image matching quality},
  author={Zhang, Zhenchao and Gerke, Markus and Vosselman, George and Yang, Michael Ying},
  journal={International journal of applied earth observation and geoinformation},
  volume={70},
  pages={25--34},
  year={2018},
}


@article{shahbazi2018high,
  title={High-density stereo image matching using intrinsic curves},
  author={Shahbazi, Mozhdeh and Sohn, Gunho and Th{\'e}au, J{\'e}rome},
  journal={ISPRS Journal of Photogrammetry and Remote Sensing},
  volume={146},
  pages={373--388},
  year={2018},}

@article{wang2020pre,
  title={Pre-Training by Completing Point Clouds},
  author={Wang, Hanchen and Liu, Qi and Yue, Xiangyu and Lasenby, Joan and Kusner, Matthew J},
  journal={arXiv preprint arXiv:2010.01089},
  year={2020}
}

@inproceedings{yuan2018pcn,
  title={{PCN}: Point completion network},
  author={Yuan, Wentao and Khot, Tejas and Held, David and Mertz, Christoph and Hebert, Martial},
  booktitle={2018 International Conference on 3D Vision (3DV)},
  pages={728--737},
  year={2018},
}

@article{jigsaw,
  title={Self-supervised deep learning on point clouds by reconstructing space},
  author={Sauder, Jonathan and Sievers, Bjarne},
  journal={Advances in Neural Information Processing Systems},
  pages={12962--12972},
  year={2019}
}

@inproceedings{xie2020pointcontrast,
  title={PointContrast: Unsupervised pre-training for 3{D} point cloud understanding},
  author={Xie, Saining and Gu, Jiatao and Guo, Demi and Qi, Charles R and Guibas, Leonidas and Litany, Or},
  booktitle={European Conference on Computer Vision},
  pages={574--591},
  year={2020},
}

@inproceedings{3DOM,
  title={a Multi-Purpose Benchmark for Photogrammetric Urban 3{D} Reconstruction in a Controlled Environment},
  author={{\"O}zdemir, Emre and Toschi, Isabella and Remondino, Fabio},
  booktitle={Evaluation and Benchmarking Sensors, Systems and Geospatial Data in Photogrammetry and Remote Sensing},
  volume={42},
  pages={53--60},
  year={2019}
}

@article{cylinder3d,
  title={Cylindrical and Asymmetrical 3{D} Convolution Networks for {LiDAR} Segmentation},
  author={Zhu, Xinge and Zhou, Hui and Wang, Tai and Hong, Fangzhou and Ma, Yuexin and Li, Wei and Li, Hongsheng and Lin, Dahua},
  journal={arXiv preprint arXiv:2011.10033},
  year={2020}
}

@article{Point_transformer,
  title={Point transformer},
  author={Zhao, Hengshuang and Jiang, Li and Jia, Jiaya and Torr, Philip and Koltun, Vladlen},
  journal={arXiv preprint arXiv:2012.09164},
  year={2020}
}

@article{SPH3D,  
  title={Spherical Kernel for Efficient Graph Convolution on 3{D} Point Clouds},  
  author={Lei, Huan and Akhtar, Naveed and Mian, Ajmal},  
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},  
  year={2020}  
}

@inproceedings{
  e3d,
  title = {Searching Efficient 3{D} Architectures with Sparse Point-Voxel Convolution},
  author = {Tang, Haotian* and Liu, Zhijian* and Zhao, Shengyu and Lin, Yujun and Lin, Ji and Wang, Hanrui and Han, Song},
  booktitle = {European Conference on Computer Vision},
  pages={685--702},
  year = {2020}
}

@inproceedings{mprm,
  title={Multi-path region mining for weakly supervised 3{D} semantic segmentation on point clouds},
  author={Wei, Jiacheng and Lin, Guosheng and Yap, Kim-Hui and Hung, Tzu-Yi and Xie, Lihua},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4384--4393},
  year={2020}
}

@inproceedings{xu2020weakly,
  title={Weakly supervised semantic point cloud segmentation: Towards 10x fewer labels},
  author={Xu, Xun and Lee, Gim Hee},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13706--13715},
  year={2020}
}


@inproceedings{simclr,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International Conference on Machine Learning},
  pages={1597--1607},
  year={2020},
}

@inproceedings{he2020momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9729--9738},
  year={2020}
}


@article{zhang2021self,
  title={Self-Supervised Pretraining of 3{D} Features on any Point-Cloud},
  author={Zhang, Zaiwei and Girdhar, Rohit and Joulin, Armand and Misra, Ishan},
  journal={arXiv preprint arXiv:2101.02691},
  year={2021}
}

@article{hou2020exploring,
  title={Exploring Data-Efficient 3{D} Scene Understanding with Contrastive Scene Contexts},
  author={Hou, Ji and Graham, Benjamin and Nie{\ss}ner, Matthias and Xie, Saining},
  journal={arXiv preprint arXiv:2012.09165},
  year={2020}
}

@article{orientation,
  title={Self-Supervised Learning of Point Clouds via Orientation Estimation},
  author={Poursaeed, Omid and Jiang, Tianxing and Qiao, Quintessa and Xu, Nayun and Kim, Vladimir G},
  journal={arXiv preprint arXiv:2008.00305},
  year={2020}
}

@article{ao2020spinnet,
  title={SpinNet: Learning a General Surface Descriptor for 3D Point Cloud Registration},
  author={Ao, Sheng and Hu, Qingyong and Yang, Bo and Markham, Andrew and Guo, Yulan},
  journal={arXiv preprint arXiv:2011.12149},
  year={2020}
}

@article{H3D,
  title={H3D: Benchmark on Semantic Segmentation of High-Resolution 3D Point Clouds and textured Meshes from UAV LiDAR and Multi-View-Stereo},
  author={K{\"o}lle, Michael and Laupheimer, Dominik and Schmohl, Stefan and Haala, Norbert and Rottensteiner, Franz and Wegner, Jan Dirk and Ledoux, Hugo},
  journal={arXiv preprint arXiv:2102.05346},
  year={2021}
}

@article{hu2020towards,
  title={Towards Semantic Segmentation of Urban-Scale 3D Point Clouds: A Dataset, Benchmarks and Challenges},
  author={Hu, Qingyong and Yang, Bo and Khalid, Sheikh and Xiao, Wen and Trigoni, Niki and Markham, Andrew},
  journal={arXiv preprint arXiv:2009.03137},
  year={2020}
}

@inproceedings{jiang2020pointgroup,
  title={Pointgroup: Dual-set point grouping for 3d instance segmentation},
  author={Jiang, Li and Zhao, Hengshuang and Shi, Shaoshuai and Liu, Shu and Fu, Chi-Wing and Jia, Jiaya},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4867--4876},
  year={2020}
}

@article{laine2016temporal,
  title={Temporal ensembling for semi-supervised learning},
  author={Laine, Samuli and Aila, Timo},
  journal={arXiv preprint arXiv:1610.02242},
  year={2016}
}

@inproceedings{MT,
  title={Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results},
  author={Tarvainen, Antti and Valpola, Harri},
  booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
  pages={1195--1204},
  year={2017}
}

@inproceedings{lei2020seggcn,
  title={{SegGCN}: Efficient 3{D} Point Cloud Segmentation With Fuzzy Spherical Kernel},
  author={Lei, Huan and Akhtar, Naveed and Mian, Ajmal},
  booktitle={CVPR},
  year={2020}
}

@article{tao2020seggroup,
  title={SegGroup: Seg-Level Supervision for 3D Instance and Semantic Segmentation},
  author={Tao, An and Duan, Yueqi and Wei, Yi and Lu, Jiwen and Zhou, Jie},
  journal={arXiv preprint arXiv:2012.10217},
  year={2020}
}

@article{shi2021label_effcient,
  title={Label-Efficient Point Cloud Semantic Segmentation: An Active Learning Approach},
  author={Shi, Xian and Xu, Xun and Chen, Ke and Cai, Lile and Foo, Chuan Sheng and Jia, Kui},
  journal={arXiv preprint arXiv:2101.06931},
  year={2021}
}

@article{Canonical_Capsules,
  title={Canonical Capsules: Unsupervised Capsules in Canonical Pose},
  author={Sun, Weiwei and Tagliasacchi, Andrea and Deng, Boyang and Sabour, Sara and Yazdani, Soroosh and Hinton, Geoffrey and Yi, Kwang Moo},
  journal={arXiv preprint arXiv:2012.04718},
  year={2020}
}

@article{self_few_shot,
  title={Self-Supervised Few-Shot Learning on Point Clouds},
  author={Sharma, Charu and Kaul, Manohar},
  journal={arXiv preprint arXiv:2009.14168},
  year={2020}
}

@article{liu2020p4contrast,
  title={P4Contrast: Contrastive Learning with Pairs of Point-Pixel Pairs for RGB-D Scene Understanding},
  author={Liu, Yunze and Yi, Li and Zhang, Shanghang and Fan, Qingnan and Funkhouser, Thomas and Dong, Hao},
  journal={arXiv preprint arXiv:2012.13089},
  year={2020}
}


% Fang
@article{cheng20212,
  title={{2-S3Net}: Attentive Feature Fusion with Adaptive Feature Selection for Sparse Semantic Segmentation Network},
  author={Cheng, Ran and Razani, Ryan and Taghavi, Ehsan and Li, Enxu and Liu, Bingbing},
  journal={arXiv preprint arXiv:2102.04530},
  year={2021}
}

@article{yan2020sparse,
  title={Sparse Single Sweep LiDAR Point Cloud Segmentation via Learning Contextual Shape Priors from Scene Completion},
  author={Yan, Xu and Gao, Jiantao and Li, Jie and Zhang, Ruimao and Li, Zhen and Huang, Rui and Cui, Shuguang},
  journal={arXiv preprint arXiv:2012.03762},
  year={2020}
}

@inproceedings{aksoy2019salsanet,
  title={Salsanet: Fast road and vehicle segmentation in lidar point clouds for autonomous driving},
  author={Aksoy, Eren Erdal and Baci, Saimir and Cavdar, Selcuk},
  booktitle={IEEE Intelligent Vehicles Symposium (IV)},
  pages={926--932},
  year={2019}
  }



@inproceedings{kundu2020virtual,
  title={Virtual multi-view fusion for 3d semantic segmentation},
  author={Kundu, Abhijit and Yin, Xiaoqi and Fathi, Alireza and Ross, David and Brewington, Brian and Funkhouser, Thomas and Pantofaru, Caroline},
  booktitle={European Conference on Computer Vision},
  pages={518--535},
  year={2020},
  organization={Springer}
}

@inproceedings{feihu,
  title={Deep fusionnet for point cloud semantic segmentation},
  author={Zhang, Feihu and Fang, Jin and Wah, Benjamin and Torr, Philip},
  booktitle={ECCV},
  volume={2},
  pages={6},
  year={2020}
}

@inproceedings{jaritz2019multi,
  title={Multi-view pointnet for 3d scene understanding},
  author={Jaritz, Maximilian and Gu, Jiayuan and Su, Hao},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision Workshops},
  pages={0--0},
  year={2019}
}


@article{wang2020weakly,
  title={Weakly Supervised Semantic Segmentation in 3D Graph-Structured Point Clouds of Wild Scenes},
  author={Wang, Haiyan and Rong, Xuejian and Yang, Liang and Feng, Jinglun and Xiao, Jizhong and Tian, Yingli},
  journal={arXiv preprint arXiv:2004.12498},
  year={2020}
}

@inproceedings{wang2019towards,
  title={Towards Weakly Supervised Semantic Segmentation in 3D Graph-Structured Point Clouds of Wild Scenes.},
  author={Wang, Haiyan and Rong, Xuejian and Yang, Liang and Wang, Shuihua and Tian, Yingli},
  booktitle={BMVC},
  pages={284},
  year={2019}
}

@inproceedings{thabet2020self,
  title={Self-supervised learning of local features in 3d point clouds},
  author={Thabet, Ali and Alwassel, Humam and Ghanem, Bernard},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={938--939},
  year={2020}
}

@inproceedings{cam,
  title={Learning deep features for discriminative localization},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2921--2929},
  year={2016}
}

@inproceedings{densecrf,
  title={Efficient inference in fully connected CRFs with Gaussian edge potentials},
  author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
  booktitle={Proceedings of the 24th International Conference on Neural Information Processing Systems},
  pages={109--117},
  year={2011}
}
